Dark Energy Survey Year 3 Results: Cosmology from Cosmic Shear and Robustness to Data Calibration

This work, together with its companion paper, Secco and Samuroff et al. (2021), presents the Dark Energy Survey Year 3 cosmic shear measurements and cosmological constraints based on an analysis of over 100 million source galaxies. With the data spanning 4143 deg$^2$ on the sky, divided into four redshift bins, we produce the highest significance measurement of cosmic shear to date, with a signal-to-noise of 40. We conduct a blind analysis in the context of the $\Lambda$CDM model and find a 3% constraint of the clustering amplitude, $S_8\equiv \sigma_8 (\Omega_{\rm m}/0.3)^{0.5} = 0.759^{+0.025}_{-0.023}$. A $\Lambda$CDM-Optimized analysis, which safely includes smaller scale information, yields a 2% precision measurement of $S_8= 0.772^{+0.018}_{-0.017}$ that is consistent with the fiducial case. The two low-redshift measurements are statistically consistent with the Planck Cosmic Microwave Background result, however, both recovered $S_8$ values are lower than the high-redshift prediction by $2.3\sigma$ and $2.1\sigma$ ($p$-values of 0.02 and 0.05), respectively. The measurements are shown to be internally consistent across redshift bins, angular scales and correlation functions. The analysis is demonstrated to be robust to calibration systematics, with the $S_8$ posterior consistent when varying the choice of redshift calibration sample, the modeling of redshift uncertainty and methodology. Similarly, we find that the corrections included to account for the blending of galaxies shifts our best-fit $S_8$ by $0.5\sigma$ without incurring a substantial increase in uncertainty. We examine the limiting factors for the precision of the cosmological constraints and find observational systematics to be subdominant to the modeling of astrophysics. Specifically, we identify the uncertainties in modeling baryonic effects and intrinsic alignments as the limiting systematics.

==> DES cosmic shear 1/commands.tex <==
\usepackage{soul} 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xspace}
\usepackage[dvipsnames]{xcolor}

% General formatting
\newcommand{\ie}{i.e.\xspace}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\etc}{etc.\xspace}
\newcommand{\etal}{et al.\xspace}
\newcommand{\vs}{vs.\xspace}
\newcommand{\super}[1]{\ensuremath{^{\textrm{#1}}}}
\newcommand{\sub}[1]{\ensuremath{_{\textrm{#1}}}}

% Todo comments
\newcommand{\FIXME}[1]{{\bf \textcolor{red}{#1}}}
%\newcommand{\FIXME}[1]{{}}
\newcommand{\CHECK}[1]{{\textcolor{orange}{#1}}}
%\newcommand{\CHECK}[1]{{#1}}
\newcommand{\COMMENT}[3]{{\textcolor{#1}{(#2: #3)}}}
%\newcommand{\COMMENT}[3]{{}}
\newcommand{\NOTE}[1]{\COMMENT{blue}{}{#1}}
\newcommand{\NEW}[1]{\COMMENT{blue}{}{#1}}

\newcommand{\XX}{{\color{red}{XX}}\xspace}
%\newcommand{\XX}{\COMMENT{red}{XX}{}}
%\newcommand\todo[1]{\todo[color=red, inline, size=\small]{TO DO: #1}}

\newcommand{\todo}[1]{\COMMENT{magenta}{TBD}{#1}}
\newcommand{\later}[1]{\COMMENT{red}{TBD}{#1}}
%\newcommand{\cd}[1]{\textcolor{Dandelion}{#1}\xspace}

\newcommand{\sd}[1]{\COMMENT{blue}{SD}{#1}}
\newcommand{\amon}[1]{\COMMENT{blue}{AA}{#1}}
\newcommand{\cd}[1]{\COMMENT{Dandelion}{CD}{#1}}
\newcommand{\NM}[1]{\textcolor{Purple}{NM: #1}\xspace}
\newcommand{\AC}[1]{\COMMENT{teal}{AC}{#1}}
\newcommand{\ACed}[1]{\textcolor{teal}{#1}}

% Units
\newcommand{\unit}[1]{\ensuremath{\mathrm{\,#1}}\xspace}
\newcommand{\Gyr}{\unit{Gyr}}
\newcommand{\eV}{\unit{eV}}
\newcommand{\keV}{\unit{keV}}
\newcommand{\MeV}{\unit{MeV}}
\newcommand{\GeV}{\unit{GeV}}
\newcommand{\TeV}{\unit{TeV}}
\newcommand{\MB}{\unit{MB}}
\newcommand{\GB}{\unit{GB}}
\newcommand{\TB}{\unit{TB}}
\newcommand{\degree}{\ensuremath{{}^{\circ}}\xspace}
\newcommand{\mas}{\unit{mas}}
\newcommand{\amin}{\unit{arcmin}}
%\newcommand{\asec}{\unit{arcsec}}
\newcommand{\angstrom}{\unit{\AA}}
\newcommand{\um}{\unit{$\mu$m}}
\newcommand{\cm}{\unit{cm}}
\newcommand{\km}{\unit{km}}
\newcommand{\kms}{\km \second^{-1}}
\newcommand{\pc}{\unit{pc}}
\newcommand{\kpc}{\unit{kpc}}
\newcommand{\second}{\unit{s}}
\newcommand{\us}{\unit{$\mu$s}}
\newcommand{\photons}{\unit{ph}}
\newcommand{\photon}{\unit{ph}}
\newcommand{\sr}{\unit{sr}}
\newcommand{\Msolar}{\unit{M_\odot}}
\newcommand{\Msun}{\unit{M_\odot}}
\newcommand{\Mstar}{\unit{M_{*}}}
\newcommand{\Lsolar}{\unit{L_\odot}}
\newcommand{\Lsun}{\unit{L_\odot}}
\newcommand{\Lstar}{\unit{L_{*}}}
\newcommand{\Lum}{\ensuremath{ L }\xspace}
\newcommand{\Dsun}{\unit{D_\odot}}
\newcommand{\cmcubes}{\ensuremath{\cm^{3}\second^{-1}}\xspace}
\newcommand{\magn}{\unit{mag}}
\newcommand{\mmag}{\unit{mmag}}
\newcommand{\e}{\unit{e^{-}}}
\newcommand{\rms}{\unit{rms}}
\newcommand{\pix}{\unit{pix}}
\newcommand{\rmspix}{\unit{rms/pix}}
\newcommand{\ermspix}{\e \rmspix}

% Referencing 
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\eqnref}[1]{Equation~\eqref{eqn:#1}}

\newcommand{\secrefs}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\tabrefs}[2]{Tables~\ref{tab:#1} and \ref{tab:#2}}
\newcommand{\figrefs}[2]{Figures~\ref{fig:#1} and \ref{fig:#2}}

% Code and variables
\newcommand{\code}[1]{\textsc{#1}\xspace}
\newcommand{\sx}{\code{SExtractor}}
\newcommand{\psfex}{\code{PSFEx}}
\newcommand{\ngmix}{\code{ngmix}}
\newcommand{\galsim}{\code{Galsim}}
\newcommand{\buzzard}{\code{Buzzard v2.0}}
\newcommand{\hyperrank}{\code{hyperrank}}

\newcommand{\bandvar}[2][]{%
  \ifthenelse{\isempty{#1}}{\var{#2}}{\var{#2\_#1}}%
}
\newcommand{\spreadmodel}[1][]{\bandvar[#1]{spread\_model}}
\newcommand{\spreaderrmodel}[1][]{\bandvar[#1]{spreaderr\_model}}
\newcommand{\wavgspreadmodel}[1][]{\bandvar[#1]{wavg\_spread\_model}}
\newcommand{\classstar}[1][]{\bandvar[#1]{class\_star}}
\newcommand{\magauto}[1][]{\bandvar[#1]{mag\_auto}}
\newcommand{\magpsf}[1][]{\bandvar[#1]{mag\_psf}}
\newcommand{\magerrpsf}[1][]{\bandvar[#1]{magerr\_psf}}
\newcommand{\flags}[1][]{\bandvar[#1]{flags}}

% DES physics
\newcommand{\LCDM}{\ensuremath{\rm \Lambda CDM}\xspace}
%\newcommand{\lcdm}{\Lambda CDM\xspace}
\newcommand{\lcdm}{\LCDM}

\newcommand{\mcal}{\textsc{Metacalibration}\xspace}
\newcommand{\mcalR}{\mbox{\boldmath $R$}}
\newcommand{\mcalRtwo}{\mbox{\boldmath $R^{\rm 2pt}$}}
\newcommand{\mcalRg}{\mbox{\boldmath $R_\gamma$}}
\newcommand{\mcalRs}{\mbox{\boldmath $R_{\rm s}$}}
\newcommand{\sompz}{\textsc{SOMPZ}\xspace}
\newcommand{\WZ}{\textsc{WZ}\xspace}
\newcommand{\SR}{\textsc{SR}\xspace}
\newcommand{\SPC}{\textsc{SPC}\xspace}
\newcommand{\PC}{\textsc{PC}\xspace}
\newcommand{\SC}{\textsc{SC}\xspace}
\newcommand{\C}{\textsc{C}\xspace}
\newcommand{\SPCMB}{\textsc{SPC-MB}\xspace}
\newcommand{\Spec}{\textsc{S}\xspace}

\newcommand{\inprep}{\emph{in preparation}\xspace}
\newcommand{\snr}{S/N\xspace}

\newcommand{\est}{e}
\newcommand{\pp}{\mbox{\boldmath $p$}}
\newcommand{\vesta}{\mbox{\boldmath $e_{\alpha}$}}
\newcommand{\vestb}{\mbox{\boldmath $e_{\beta}$}}
\newcommand{\vest}{\mbox{\boldmath $e$}}
\newcommand{\vwst}{\mbox{\boldmath $w$}}
\newcommand{\vqst}{\mbox{\boldmath $q$}}
\newcommand{\vecg}{\mbox{\boldmath $\gamma$}}
\newcommand{\vecc}{\mbox{\boldmath $c$}}
\newcommand{\vecgest}{\mbox{\boldmath $\gamma^{\mathrm{est}}$}}
\newcommand{\xip}{\xi_+\xspace}
\newcommand{\xim}{\xi_-\xspace}
\newcommand{\xipm}{\xi_\pm\xspace}
\newcommand{\gammat}{\gamma_{\rm t}\xspace}
\newcommand{\wtheta}{w(\theta)\xspace}
\newcommand{\kmsMpc}{\,{\rm km/s/Mpc}}



==> DES cosmic shear 1/cs1_author_list2.tex <==
% Author list file generated with: mkauthlist 1.2.4+6.g9cbd239 
% mkauthlist --sort --aux shearorder.csv DES-2019-0479_author_list.csv cs1_author_list2.tex 

\author{A.~Amon}\email{amon2018@stanford.edu}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{D.~Gruen}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{M.~A.~Troxel}
\affiliation{Department of Physics, Duke University Durham, NC 27708, USA}
\author{N.~MacCrann}
\affiliation{Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK}
\author{S.~Dodelson}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\author{A.~Choi}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{C.~Doux}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{L.~F.~Secco}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{S.~Samuroff}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\author{E.~Krause}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\author{J.~Cordero}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
\author{J.~Myles}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{J.~DeRose}
\affiliation{Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA}
\author{R.~H.~Wechsler}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{M.~Gatti}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{A. Navarro-Alsina}
\affiliation{Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{G.~M.~Bernstein}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{B.~Jain}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{J.~Blazek}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Institute of Physics, Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland}
\author{A.~Alarcon}
\affiliation{Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA}
\author{A.~Fert\'e}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{P.~Lemos}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\affiliation{Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
\author{M.~Raveri}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{A.~Campos}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\author{J.~Prat}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\author{C.~S{\'a}nchez}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{M.~Jarvis}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{O.~Alves}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{F.~Andrade-Oliveira}
\affiliation{Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{E.~Baxter}
\affiliation{Department of Physics and Astronomy, Watanabe 416, 2505 Correa Road, Honolulu, HI 96822}
\author{K.~Bechtol}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{M.~R.~Becker}
\affiliation{Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA}
\author{S.~L.~Bridle}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
\author{H.~Camacho}
\affiliation{Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{A.~Carnero~Rosell}
\affiliation{Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Universidad de La Laguna, Dpto. Astrofísica, E-38206 La Laguna, Tenerife, Spain}
\author{M.~Carrasco~Kind}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\author{R.~Cawthon}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{C.~Chang}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{R.~Chen}
\affiliation{Department of Physics, Duke University Durham, NC 27708, USA}
\author{P.~Chintalapati}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{M.~Crocce}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{C.~Davis}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{H.~T.~Diehl}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{A.~Drlica-Wagner}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{K.~Eckert}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{T.~F.~Eifler}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{J.~Elvin-Poole}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{S.~Everett}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{X.~Fang}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\author{P.~Fosalba}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{O.~Friedrich}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\author{E.~Gaztanaga}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{G.~Giannini}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra, Spain}
\author{R.~A.~Gruendl}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\author{I.~Harrison}
\affiliation{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
\author{W.~G.~Hartley}
\affiliation{Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland}
\author{K.~Herner}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{H.~Huang}
\affiliation{Department of Physics, University of Arizona, Tucson, AZ 85721, USA}
\author{E.~M.~Huff}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{D.~Huterer}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{N.~Kuropatkin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{P.~Leget}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{A.~R.~Liddle}
\affiliation{Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK}
\affiliation{Instituto de Astrof\'{\i}sica e Ci\^{e}ncias do Espa\c{c}o, Faculdade de Ci\^{e}ncias, Universidade de Lisboa, 1769-016 Lisboa, Portugal}
\affiliation{Perimeter Institute for Theoretical Physics, 31 Caroline St. North, Waterloo, ON N2L 2Y5, Canada}
\author{J.~McCullough}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{J.~Muir}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{S.~Pandey}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{Y.~Park}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo, Chiba 277-8583, Japan}
\author{A.~Porredon}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{A.~Refregier}
\affiliation{Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland}
\author{R.~P.~Rollins}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
\author{A.~Roodman}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{R.~Rosenfeld}
\affiliation{ICTP South American Institute for Fundamental Research\\ Instituto de F\'{\i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{A.~J.~Ross}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{E.~S.~Rykoff}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{J.~Sanchez}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{I.~Sevilla-Noarbe}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{E.~Sheldon}
\affiliation{Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA}
\author{T.~Shin}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{A.~Troja}
\affiliation{ICTP South American Institute for Fundamental Research\\ Instituto de F\'{\i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{I.~Tutusaus}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{I.~Tutusaus}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{T.~N.~Varga}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affiliation{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
\author{N.~Weaverdyck}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{B.~Yanny}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{B.~Yin}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\author{Y.~Zhang}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{J.~Zuntz}
\affiliation{Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK}
\author{M.~Aguena}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{S.~Allam}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{J.~Annis}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{D.~Bacon}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{E.~Bertin}
\affiliation{CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
\affiliation{Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, France}
\author{S.~Bhargava}
\affiliation{Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
\author{D.~Brooks}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{E.~Buckley-Geer}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{D.~L.~Burke}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{J.~Carretero}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra, Spain}
\author{M.~Costanzi}
\affiliation{Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy}
\affiliation{INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy}
\affiliation{Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy}
\author{L.~N.~da Costa}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~E.~S.~Pereira}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{J.~De~Vicente}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{S.~Desai}
\affiliation{Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India}
\author{J.~P.~Dietrich}
\affiliation{Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}
\author{P.~Doel}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{I.~Ferrero}
\affiliation{Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway}
\author{B.~Flaugher}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{J.~Frieman}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{J.~Garc\'ia-Bellido}
\affiliation{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\author{E.~Gaztanaga}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{D.~W.~Gerdes}
\affiliation{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{T.~Giannantonio}
\affiliation{Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\author{J.~Gschwend}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{G.~Gutierrez}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{S.~R.~Hinton}
\affiliation{School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia}
\author{D.~L.~Hollowood}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{K.~Honscheid}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{B.~Hoyle}
\affiliation{Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\author{D.~J.~James}
\affiliation{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}
\author{R.~Kron}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{K.~Kuehn}
\affiliation{Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia}
\affiliation{Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA}
\author{O.~Lahav}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{M.~Lima}
\affiliation{Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, 05314-970, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{H.~Lin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{M.~A.~G.~Maia}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{J.~L.~Marshall}
\affiliation{George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
\author{P.~Martini}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Radcliffe Institute for Advanced Study, Harvard University, Cambridge, MA 02138}
\author{P.~Melchior}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\author{F.~Menanteau}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\author{R.~Miquel}
\affiliation{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra, Spain}
\author{J.~J.~Mohr}
\affiliation{Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\author{R.~Morgan}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{R.~L.~C.~Ogando}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{A.~Palmese}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{F.~Paz-Chinch\'{o}n}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\author{D.~Petravick}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{A.~Pieres}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{A.~K.~Romer}
\affiliation{Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
\author{E.~Sanchez}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{V.~Scarpine}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{M.~Schubnell}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{S.~Serrano}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, 08193 Barcelona, Spain}
\author{M.~Smith}
\affiliation{School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK}
\author{M.~Soares-Santos}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{G.~Tarle}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{D.~Thomas}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{C.~To}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{J.~Weller}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affiliation{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}


\collaboration{DES Collaboration}


==> DES cosmic shear 1/des_acknowledgements.tex <==
Funding for the DES Projects has been provided by the U.S. Department of Energy, the U.S. National Science Foundation, the Ministry of Science and Education of Spain, 
the Science and Technology Facilities Council of the United Kingdom, the Higher Education Funding Council for England, the National Center for Supercomputing 
Applications at the University of Illinois at Urbana-Champaign, the Kavli Institute of Cosmological Physics at the University of Chicago, 
the Center for Cosmology and Astro-Particle Physics at the Ohio State University,
the Mitchell Institute for Fundamental Physics and Astronomy at Texas A\&M University, Financiadora de Estudos e Projetos, 
Funda{\c c}{\~a}o Carlos Chagas Filho de Amparo {\`a} Pesquisa do Estado do Rio de Janeiro, Conselho Nacional de Desenvolvimento Cient{\'i}fico e Tecnol{\'o}gico and 
the Minist{\'e}rio da Ci{\^e}ncia, Tecnologia e Inova{\c c}{\~a}o, the Deutsche Forschungsgemeinschaft and the Collaborating Institutions in the Dark Energy Survey. 

The Collaborating Institutions are Argonne National Laboratory, the University of California at Santa Cruz, the University of Cambridge, Centro de Investigaciones Energ{\'e}ticas, 
Medioambientales y Tecnol{\'o}gicas-Madrid, the University of Chicago, University College London, the DES-Brazil Consortium, the University of Edinburgh, 
the Eidgen{\"o}ssische Technische Hochschule (ETH) Z{\"u}rich, 
Fermi National Accelerator Laboratory, the University of Illinois at Urbana-Champaign, the Institut de Ci{\`e}ncies de l'Espai (IEEC/CSIC), 
the Institut de F{\'i}sica d'Altes Energies, Lawrence Berkeley National Laboratory, the Ludwig-Maximilians Universit{\"a}t M{\"u}nchen and the associated Excellence Cluster Universe, 
the University of Michigan, NFS's NOIRLab, the University of Nottingham, The Ohio State University, the University of Pennsylvania, the University of Portsmouth, 
SLAC National Accelerator Laboratory, Stanford University, the University of Sussex, Texas A\&M University, and the OzDES Membership Consortium.

Based in part on observations at Cerro Tololo Inter-American Observatory at NSF's NOIRLab (NOIRLab Prop. ID 2012B-0001; PI: J. Frieman), which is managed by the Association of Universities for Research in Astronomy (AURA) under a cooperative agreement with the National Science Foundation.

The DES data management system is supported by the National Science Foundation under Grant Numbers AST-1138766 and AST-1536171.
The DES participants from Spanish institutions are partially supported by MICINN under grants ESP2017-89838, PGC2018-094773, PGC2018-102021, SEV-2016-0588, SEV-2016-0597, and MDM-2015-0509, some of which include ERDF funds from the European Union. IFAE is partially funded by the CERCA program of the Generalitat de Catalunya.
Research leading to these results has received funding from the European Research
Council under the European Union's Seventh Framework Program (FP7/2007-2013) including ERC grant agreements 240672, 291329, and 306478.
We  acknowledge support from the Brazilian Instituto Nacional de Ci\^encia
e Tecnologia (INCT) do e-Universo (CNPq grant 465376/2014-2).

This manuscript has been authored by Fermi Research Alliance, LLC under Contract No. DE-AC02-07CH11359 with the U.S. Department of Energy, Office of Science, Office of High Energy Physics.

==> DES cosmic shear 1/extra_notneeded/abe/psfextra.tex <==
\begin{comment}
\begin{center} 
 \centering 
 \begin{table}
 \begin{tabular}{ ccccc} \hline 
 & Bin 1 & Bin 2 & Bin 3 & Bin 4 \\ \hline \rule{0pt}{3ex} 
 $\alpha$ & $0.019_{-0.003}^{+0.003}$ & $0.017_{-0.004}^{+0.004}$ & $0.013_{-0.004}^{+0.004}$ & $0.029_{-0.005}^{+0.005}$\\ \rule{0pt}{3ex} 
 $\beta$ & $0.9_{-0.2}^{+0.2}$ & $1.8_{-0.2}^{+0.2}$ & $2.3_{-0.2}^{+0.2}$ & $1.6_{-0.3}^{+0.3}$ \\ \rule{0pt}{3ex} 
 $\eta$ & $-1.8_{-2.3}^{+2.4}$ & $-5.8_{-2.6}^{+2.7}$ & $1.8_{-2.6}^{+2.6}$ & $2.8_{-3.4}^{+3.2}$ \\  \rule{0pt}{3ex} 
 $\chi^{2}$ & $147.0$ & $209.4$ & $203.4$ & $213.0$ \\ 
 $\chi^{2}_{\nu}$ & $1.3$ & $1.8$ & $1.7$ & $1.8$ \\ \hline 
 \end{tabular}
 \label{tab:abe}
 \caption{The values of the parameters $\alpha$,$\beta$ and $\eta$ for each redshift bin, estimated from fits to the mean-substracted $\rho$-statistics, according to equation~\ref{eq:psf}, as well as the (reduced) goodness-of-fit, $\chi^{2}$ ($\chi^{2}_{\nu}$) for $\nu=117$ degrees of freedom. }
 \end{table}
\end{center}
\end{comment}


\begin{comment}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{abe/figs/tau0_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau1_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau2_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau3_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau4_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau5_bestfit.png}
\caption{Best fits of model $\rho(\theta)$ to data $\tau(\theta)$ for the four different redshift bins}
\label{fig:taubestfits}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{abe/figs/xipcont_xipfid_abe_1sig.png}
\includegraphics[width=0.4\textwidth]{abe/figs/ximcont_ximfid_abe_1sig.png}
\caption{\label{fig:xipbias} Comparison of the bias of the shear 2PCF due to PSF additive errors $\delta \xi^{\textrm{PSF}}$ with fiducial 2PCF $\xi$  }
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_a.png}
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_b.png}
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_c.png}
\caption{Bias of the shear two-point correlation function in terms of different diagnostics equations }
\caption{\label{fig:rhoscontribution}}
\end{figure}
\end{comment}





%For the $i$-th redshift bin, is expanded to
\begin{comment}
\begin{align}
\label{eq:2pcfbias}
\xi_{\textrm{obs}}^{ij'} &= \xi_{+ t}^{ij'} + \alpha^{i}\alpha^{j} \rho_{0} + \beta^{i}\beta^{j} \rho_{1} + \eta^{i}\eta^{j}\rho_{3} \\
&+ \left(\beta^{i}\alpha^{j} + \beta^{j}\alpha^{i}\right)\rho_{2}+
 \left( \alpha^{i}\eta^{j}+\alpha^{j}\eta^{i} \right)\rho_{5} \\
 &+ \left(\beta^{i}\eta^{j}+\beta^{j}\eta^{i} \right)\rho_{4} 
\end{align}

\end{comment}
%To find this parameters we define the likelihood function
%\begin{equation}
%\mathcal{L}=|C|^{-1/2} \exp\left(-\frac{{\bf d}^T {\bf C}^{-1}{\bf d}}{2}\right),
%\label{eq:likelihoodbebq}
%\end{equation}
%where 
%\begin{equation}
%\begin{aligned}
%    \xi_{p}= \left[ \alpha\rho_{0+}'+\beta\rho_{2+}'+\eta\rho_{5+}', \alpha\rho_{0-}'+\beta\rho_{2-}'+\eta\rho_{5-}', \right.
%    \\
%    \alpha\rho_{2+}'+\beta\rho_{1+}'+\eta\rho_{4+}', \alpha\rho_{2-}'+\beta\rho_{1-}'+\eta\rho_{4-}'), 
%    \\
%    \left. \alpha\rho_{5+}'+\beta\rho_{4+}'+\eta\rho_{3+}', \alpha\rho_{5-}'+\beta\rho_{4-}'+\eta\rho_{3-}' \right],
%\end{aligned}
%\end{equation}
%\begin{equation}
%    \hat{\xi}=\left[\tau_{0+}, \tau_{0-},\tau_{2+}, \tau_{2-},\tau_{5+},\tau_{5-} \right]
%\end{equation}
%and $\bf{C}$ is the covariance matrix of the data vector $\hat{\xi}$. 
%where the $\rho$- statistics  are defined as for galaxy-star fields as $\rho_{0}=\left\langle \pp\pp \right\rangle $, $\rho_1= \left\langle \vqst \vqst \right\rangle$,  $\rho_2= \left\langle \vqst \pp \right\rangle$, $\rho_3= \left\langle \vwst \vwst \right\rangle$, $\rho_4= \left\langle \vqst \vwst \right\rangle$ and $\rho_5= \left\langle  \pp \vwst\right\rangle$. And $\tau_{0}=\left\langle \vecgest \pp\right\rangle$, $\tau_{2}=\left\langle \vecgest \vqst \right\rangle$ and $\tau_5= \left\langle \vecgest \vwst \right\rangle$. %The primed notation in $\rho(\theta)$ means mean substraction for each star field involved. The covariance matrix was obtained using Jackknife sampling. Both $\tau(\theta)$ and $\rho(\theta)$ were meausured using \code{TreeCorr} with 20 logarithmic angular bins from 0.1 arcmin to 250 arcmin.  We solve this problem once for each redshift bin, since our star field is local we need to update only the correlations involving galaxies, i.e, $\tau(\theta)$. To solve the fitting problem we sample the posterior distribution using \code{emcee} \cite{foremanmackey19}. 




==> DES cosmic shear 1/extra_notneeded/abe/table_abe_margin_eq4_Y3_03-31-20_JKmarco.tex <==
\begin{center} 
 \centering 
 \begin{table}
 \begin{tabular}{ c|c|c|c|c} \hline 
 & \textrm{Bin}1 & \textrm{Bin}2 & \textrm{Bin}3 & \textrm{Bin}4 \\ \hline \rule{0pt}{3ex} 
 $\alpha$ & $0.019_{-0.003}^{+0.003}$ & $0.017_{-0.004}^{+0.004}$ & $0.013_{-0.004}^{+0.004}$ & $0.029_{-0.005}^{+0.005}$\\ \rule{0pt}{3ex} 
 $\beta$ & $0.884_{-0.232}^{+0.230}$ & $1.757_{-0.241}^{+0.232}$ & $2.275_{-0.236}^{+0.241}$ & $1.601_{-0.270}^{+0.280}$ \\ \rule{0pt}{3ex} 
 $\eta$ & $-1.835_{-2.329}^{+2.362}$ & $-5.815_{-2.616}^{+2.656}$ & $1.860_{-2.619}^{+2.618}$ & $2.883_{-3.370}^{+3.190}$ \\  \rule{0pt}{3ex} 
 $\chi^{2}$ & $146.996$ & $209.378$ & $203.418$ & $213.038$ \\ 
 $\chi^{2}_{(\nu=117)}$ & $1.256$ & $1.790$ & $1.739$ & $1.821$ \\ \hline 

 \end{tabular}
 \label{tab:abe}
 \caption{The values of the parameters $\alpha$,$\beta$ and $\eta$ for different tomographic bins, estimated from mean-substracted $\rho(\theta)$ and cross-correlations galaxy-star $\tau(\theta)$). }
 \end{table}
\end{center}


==> DES cosmic shear 1/extra_notneeded/data.tex <==

\begin{figure*}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figs/DESY3neff.pdf}
  %\captionof{figure}{A figure}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figs/DESY3meanz.pdf}
  %\captionof{figure}{Another figure}
  \label{fig:test2}
\end{minipage}
\caption{The DES-Y3 footprint showing the variation of the number density across the sky, as determined with the \mcal catalog (left) and the variation in mean redshift of that catalog (right). Overlaid are the locations and the outline of the Y1 footprint (left) and the locations of three of the four DES Deep Fields \citep{y3-deepfields} (right, dark points; the fourth field, invisible here, is COSMOS). The catalog spans an unmasked 4143 deg$^2$ with an average number density of 5.9 arcmin$^{-2}$ and a mean redshift of 0.633. 
}
\label{fig:map}
\end{figure*}

The Dark Energy Survey (DES) has completed a six year observing program at the Cerro Tololo Inter-American Observatory (CTIO), using the 570-megapixel Dark Energy Camera  \citep{flaugher15}. Ultimately, the complete survey spans 5000 square degrees of the Southern hemisphere in the $grizY$ bands with exposure times of 90 seconds in $griz$ and 45 seconds in $Y$ \citep{des-overview}. With 10 overlapping exposures over the full wide-field area, the survey reaches a limiting magnitude of $i \sim 24$.
%\NS{FYI, it is 23.0 for Y3 for SN = 10 extended objects or 23.3 considering fixed apertures at SN = 10. For Y6 it will be closer to 23.8 and 24 respectively I think}.

This DES Year 3 (Y3)  analysis is limited to the the data acquired over the first three years of observations, from August 15, 2013  to February 12, 2016. The survey footprint spans 4946 square degrees, after masking, with a mean depth of four exposures, with depth reaching S/N $\sim10$ for extended objects up to $i_{AB}\sim23.0$ \citep{y3-gold}. The median recorded seeing (FWHM) in the $riz$ bands is  0.98, 0.89, 0.85 arcsec, respectively for the DES Y3 shape catalog. 

The DES Y3 dataset exploits a number of improvements compared to the DES Y1 catalog, including updates in sky-background modeling, better morphological star-galaxy classification and astrometric solutions, reduced photometric residuals compared to Gaia with photometric calibration uniformity down to $< 3$ mmag, the introduction of  per-object chromatic corrections and improvements to the Point-Spread Function (PSF) modelling \citep{y3-piff} and better flagging of imaging artifacts. These improvements, as well as the production and validation of a `Gold’ catalogue of 390 million objects prior are described in detail in \citet{y3-gold}.
\begin{comment}
\begin{table*}
    \caption{c terms. }  
\label{tab:datastats}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{ccc|cc|cc|cc|cc}
%\hline 
Bin $\times 10^{-4}$& $ w e_1 $  & $w e_2 $ & $e_1 $  & $e_2 $ & Y1 $e_1$ & Y1 $e_2$&  Y3, Y1 area $e_1$&  Y3, Y1 area $e_2$ &  Y3, Y1 area $w e_1$&  Y3, Y1 area $w  e_2$    \tabularnewline
\hline 

0 & 3.22 & 1.60 & 3.50 & 1.58 & 0.8 & 4.3 & 2.76 & 1.87 \tabularnewline
1 & 3.36 & 0.38 & 3.51 & 0.77  & 1.6 & 4.5& 2.35 & 1.26 \tabularnewline
2 & 3.77 & 0.07 & 3.94 & 0.29 & 3.8 & -2.0 & 3.59 & -1.55 \tabularnewline
3 & 4.06 & -0.27 & 4.54 & -0.06 & 8.9 & -1.7 & 4.85 & -1.36 \tabularnewline
%\hline 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table*}
\end{comment}



\subsection{Shape measurement}
%\label{sect:cat_selection}
Shape measurement can be summarised with a first-order approximation of the observed ellipticity or shear estimator, $\epsilon^{\rm obs}$, of the form
\begin{equation}
\label{eqn:shearbias}
    \epsilon^{\rm obs} = (1+m)(\epsilon^{\rm int} + \gamma) + c\, ,
\end{equation}
where the intrinsic ellipticity of the galaxy, $\epsilon^{\rm int}$ has an additional cosmic shear, $\gamma$, as well as an additive bias, $c$, and multiplictive bias, $m$.

For the DES Y3 analysis, \mcal is used to produce the shear catalog \citep{SheldonMcal2017, Huff_Mandelbaum_2017}. This method calibrates shear statistics, such as a mean shear estimate or the shear two-point function, from available imaging data, without reliance on prior information about galaxy properties. 
It measures the ellipticity using a single Gaussian model that is fit to each detected object, for all the available epochs, using the $riz$-band images (the $g$-band is excluded in the fit due to insufficient PSF modeling, as detailed in \citet{y3-piff}). During the fit, light from neighbouring objects is masked in order to reduce blending effects. The galaxy image is then deconvolved with the PSF, artificially sheared, reconvolved by a symmetrized version of the PSF and the ellipticity remeasured. Done repeatedly, this results in one unsheared and four sheared versions of the shape catalog (one for each direction ($\pm$) and component of shear), each of which include unique flux measurements, to construct the shear response matrix, \mcalRg, via numerical derivatives of the ellipticity.  The response matrix is a noisy quantity on a single galaxy basis, but ensemble averages are unbiased and known to a high degree of accuracy given the size of the DES Y3 sample. The pipeline is largely based upon that used in the DES Y1 analysis the inclusion of an inverse variance weighting for the galaxies, employed to boost the signal-to-noise of the data. The details of this implementation can be found in \citet{y3-shapecatalog}. 

The \mcal\ pipeline is designed to self-calibrate biases in the shear estimation by correcting for not only the response of the shear estimator, but also the selection biases \citep{Huff_Mandelbaum_2017}. The artificially sheared versions of each original galaxy image are used to compute the shear response matrix, using a central finite difference estimate. Selection biases can be corrected for by selecting objects on sheared measurements and computing a selection response, \mcalRs,  as, 
 \begin{eqnarray}
\left<\mcalRs_{i,j} \right>  = \frac{\left< e_i\right>^{S_+}-\left< e_i\right>^{S_-}}{\Delta \gamma_j} \, ,
\end{eqnarray}
where $\left<e_i\right>^{S_+}$ represents the mean of the $i$th ellipticity component measured on images without applied shearing in component $j$, over the group of galaxies selected using the parameters extracted from positively sheared images. $\left<e_i\right>^{S_-}$ is the analogue quantity for negatively sheared images. To calibrate the mean shear of the catalog, it is sufficient to consider the total response matrix:
\begin{eqnarray}
\label{eqn:response}
\left<\boldsymbol{R} \right> =  \left<\boldsymbol{R}_\gamma \right> + \left<\boldsymbol{R}_S \right> \, .
\end{eqnarray}
 The response matrix is diagonal, within a very good approximation and as a consequence, the mean shear response correction reduces to element-wise division. The \mcal\ response accounts for shear biases at a level of a few parts in a thousand in absence of blends and detection biases \citep{SheldonMcal2017}.  The current \mcal\ implementation, however, does not correct for a shear-dependent detection bias \citep{metadetect}, which leaves a multiplicative factor at the level of $m\sim2-3$\% and it is calibrated using image simulations in \citep{y3-imagesims} and discussed in Section~\ref{sec:imsims}. 



\subsection{DES Y3 weak lensing catalog and validation}

Only objects that pass a number of criteria are included in the weak lensing selection. This is encoded in a \texttt{INDEX/SELECT} column in the catalog and encompasses selections based on a combination of galaxy and PSF properties, which are designed to reduce potential systematic biases due to, for example blending, PSF mis-estimation and stellar contamination. In addition, magnitude selections are imposed ($i=18-23.5$ and $rz=15-26$) to limit the analysis to include only galaxies with robust redshift estimation. Finally, we limit our study to objects that are contained within the redMaGiC mask, bringing the footprints' final effective area to span $A_{\rm eff}= 4143$ deg$^2$.  The resulting \mcal\ catalog yields 100 202 538 objects, with a weighted number density of $n_{\rm eff}=5.90$ galaxies arcmin$^{-2}$, as defined by \cite{Heymans13}, spanning a final area of $A_{\rm eff}= 4143$ deg$^2$ . Table~\ref{tab:datastats} lists the effective number density for the full catalog and the corresponding weighted ellipticity variance.  The statistical power of the \mcal\ catalog without galaxy weights is tripled compared to Y1, with weighting increasing this further by $\approx 25\%$ \cite{y3-shapecatalog}. 

The spatial variation of number density over the survey footprint is shown in the left-hand panel of Figure~\ref{fig:map} with a map that utilises \texttt{SKYMAPPER}\footnote{https://github.com/kadrlica/skymap} in \textsc{HEALPIX} cells of nside=1024. Overlaid are the bounds of the previous DES Y1 and SV surveys.

The \mcal\ shape catalog has passed a raft of empirical tests detailed in \citet{y3-shapecatalog}, aimed at identifying residual additive biases for the full catalog. These validated against systematic errors connected to PSF errors, which were proven to be negligible for the full catalog with a smaller amplitude compared to the DES Y1 analysis. In addition, the catalog was proven robust against the presence of spurious B-modes using two different estimators, COSEBIs and Pseudo-$C_\ell$, which consistently resulted in a null detection (see also Appendix~\ref{App:Bmodes}). In Section~\ref{sec:robustshear}, these tests are extended to the tomographic case. Further tests included checking the dependency of the two components of the shear with respect to a number of galaxy or survey properties, finding no significant correlations, except for a linear dependence between $\langle e_1 \rangle$ and the ratio between the galaxy size and PSF size. The origin of this trend is unknown, but it was verified to be safely neglected in the cosmological analysis.



 
\begin{table*}
    \caption{DES Y3 data properties per redshift bin: the unweighted number of objects passing the weak-lensing selection, the effective number density $n_{\rm eff}$ (gal/arcmin$^2$), calculated with $A_{\rm eff}= 4143$ deg$^2$, the per-component shape noise, $\sigma_e$, the mean redshift, $z_{\rm mean}$, the spread in the mean redshift of the redshift distribution realisations, $\Delta z$, the shear calibration parameter, $m$, and the mean shear per component, $c_{1,2}=\langle e_{1,2} \rangle$. }  
\label{tab:datastats}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{cccccccccccc}
%\hline 
Redshift bin & no. objects & $n_{\rm eff}$ & $\sigma_e$ &  $z_{\rm mean}$  & $\langle e_1 \rangle \times 10^{4}$  & $\langle e_2 \rangle \times 10^{4}$ & $\Delta z$& $m$ & $\Delta z_{\rm no blend}$& $m_{\rm no blend}$   \tabularnewline
\hline 
Full & 100 204 026 &5.900 & 0.268 &  0.633 &  - & -  & - & - & - & - \tabularnewline
0 & 24 941 833 & 1.476 & 0.243 & 0.336 & 3.22 & 1.60  &    0.018 & -0.006 $ \pm $ 0.009 & 0.016  & -0.013 $ \pm $ 0.003\tabularnewline
1 & 25 281 777 & 1.479 & 0.262 & 0.521 & 3.36 & 0.38 &  0.015 & -0.020 $ \pm $ 0.008 & 0.013  & -0.018 $ \pm $ 0.004\tabularnewline
2 & 24 892 990 & 1.484 &  0.259 &  0.742 & 3.77 & 0.07&  0.011 & -0.024 $ \pm $ 0.008 & 0.006  & -0.023 $ \pm $ 0.004 \tabularnewline
3 & 25 092 344 & 1.461 & 0.301 &  0.964  & 4.06 & -0.27 &  0.017 & -0.037 $ \pm $ 0.008 & 0.015  & -0.036 $ \pm $ 0.006 \tabularnewline
%\hline 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table*}

==> DES cosmic shear 1/extra_notneeded/modelling.tex <==
In this section, we outline the baseline theoretical model for the shear 2-point correlation functions used in this analysis and discuss the evidence for its robustness. That is, it is exemplified in \citep{y3-generalmethods} that systematic errors in the model are subdominant to the precision of the data, in order to derive unbiased cosmological parameters. 

For parameter inference, the likelihood, $\mathcal{L}(\textbf{p})$, is assumed to be a multivariate Gaussian in the multi-dimensional parameter space,
\begin{equation}
\ln{\mathcal{L}(\textbf{p})} = -\frac{1}{2} \sum_{ij} (D_i-T_i(\textbf{p})\,\,C^{-1}_{ij}\,\,(D_j-T_j(\textbf{p})) \,,
\end{equation}
where $\textbf{p}$ denotes the full set of parameters. The data vector, $D$, presented in Section~\ref{sec:measurement} initially contains 20 angular data points over 4 redshift bins and 2 correlation functions, which amounts to
227 data points after the limiting the angular scales, according to Section~\ref{sec:scalecuts}. $D_i$ represents the $i$th element of the data vector, comprised of the tomographic two-point correlation functions,  $\xi_{\pm}$, presented in Figure~\ref{fig:xitomo}. the corresponding theoretical prediction for the measurements,  $T_i(\textbf{p})$, are detailed in this section. The covariance matrix, $C$, summarised in Section~\ref{sec:covariance}, does depend on the model parameters $\textbf{p}$, but a fiducial set of parameters is assumed and use a fixed covariance implemented in this analysis, after an iterative process. The posteriors of the cosmological parameters are computed as the product of the likelihood with the priors, $\mathcal{P(\textbf{p})}$, listed in Table~\ref{tab:priors}. 

The likelihood is sampled with the \textsc{Polychord sampler} \cite{Handley15}. This analysis pipeline is built upon the framework \textsc{CosmoSIS} \citep{zuntz15}, a modular cosmological parameter estimation code. Although the fiducial settings (500 live points, tolerance 0.1) have been
tested to demonstrate the accuracy of the posteriors and Bayesian evidence estimates \citep[see][]{Lemos2020}, the position of the peak in 19 dimensional space is noisy. As such, point estimates, are obtained with the \textsc{MaxLike} minimizer. Validation of this aspect is achieved through redundancy in an implementation of the analysis pipeline independently in \textsc{cosmolike} \citep{Krause17,y3-generalmethods}. To calculate the linear matter power spectrum $P_{\rm NL}(k, z)$, \textsc{CosmoSIS} uses \textsc{CAMB} \citep{CAMB}.  


Cosmological, astrophysical, and systematic parameters are constrained for the $\Lambda$CDM model. For the case of cosmological parameters that are not well-constrained by cosmic shear, informative priors that widely encompass allowed values from external experiments are used. In
particular, for $\Omega_{\nu}h^2$ we take a lower limit derived from oscillation experiments [105], and an upper limit  that is roughly five times the 95\% confidence limit of the limiting value found by external data,  $\Omega_{\nu}h^2 \sim 0.002$ \citep{Planck2018}. These prior boundaries are reported in Table~\ref{tab:priors}. We leave exploration of other cosmological models to future work. In this section, we detail the fiducial cosmological model used in the analysis, as well as the modelling of the systematics. 



\subsection{Cosmic shear signal}
\begin{comment}
\begin{equation}
\centering
\xi^{ij}_{+}(\theta) = \frac{1}{2 \pi} \int d\ell \,\,\, \ell P_{\kappa}^{ij}(\ell)  \, J_{0}(\ell\theta) 
\end{equation}
\begin{equation}
\centering
P_{\kappa}^{ij}(\ell) = \int d\chi \,\,\,  Q(\chi) \, P_{\delta}\big(\frac{\ell}{\chi},\chi\big) 
\end{equation}
\end{comment}
The observed angular two-point correlation for two redshift bins, $i$ and $j$, is theoretically expressed in terms of the the convergence power spectrum, $C_{\kappa}(\ell)$, at an angular wavenumber, $\ell$, as
\begin{align}
\centering
\label{eqn:2ptP}
{}& \xi_+(\theta) = \sum_{\ell} \frac{2\ell+1}{4\pi} G^\pm_\ell(\cos \theta) \qty[C_{\kappa,\textrm{EE}}^{ij}(\ell)\pm C_{\kappa, \textrm{BB}}^{ij}(\ell)] \, , \\
& \xi_-(\theta) = \sum_{\ell} \frac{2\ell+1}{4\pi} G^\pm_\ell(\cos \theta) \qty[C_{\kappa,\textrm{EE}}^{ij}(\ell) - C_{\kappa, \textrm{BB}}^{ij}(\ell)],
\end{align}
\noindent
where the functions $G^\pm_\ell(x)$ are computed from Legendre polynomials $P_\ell(x)$ (see, e.g. \citealt{y3-covariances}, appendix A). We include the B-mode power spectra here for completeness. Although cosmological lensing does not produce B-modes, our fiducial model does include a B-mode contribution from intrinsic alignments, and so we show the more general expression here.  

The 2D convergence power spectrum, $C_{\kappa}$, can be related to the non-linear 3D matter power spectrum, $P_{\delta}$, via a simplification with a flat-sky and  the Limber approximation \citep{Limber53,Limber_LoVerde2008}.  These approximations begin to break down for small $\ell$-modes. The applicability of these approximations and corrections are investigated in \citet{Kilbinger17} and \cite{Kitching17} and a `hybrid' case, used in most recent cosmic shear analyses, can be written as, 
\begin{equation}
\centering
C_{\kappa}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{W_i(\chi)W_j(\chi)}{\chi^2}  P_{\delta}\left(k=\frac{\ell+0.5}{z(\chi)},\chi\right) \, ,
\end{equation}\label{eq:limber_gg}
\noindent
where $\chi_{\rm H}$ is the horizon distance and a flat spatial geometry is assumed, so that $f_K(\chi)$, the comoving angular diameter distance, is simplified to $\chi$. The lensing efficiency kernel, $W_i(\chi)$, for the tomographic bin $i$ is defined as,
\begin{equation}
\label{eqn:kernel}
\centering
W_i(\chi)= \frac{3H_0^2\Omega_{\rm m}}{2c^2}\frac{\chi}{a(\chi)} \int_{\chi}^{\chi_{\rm H}} d\chi' \, \tilde{n}_i(\chi') \frac{\chi'-\chi}{\chi'}  \, ,
\end{equation}
\noindent
where $\tilde{n}_i(\chi) d\chi$ is the effective number of galaxies in $d\chi$ in the $i$th redshift bin, normalised such that $\int_{\chi}^{\chi_{\rm H}} \tilde{n}_i(\chi) d\chi =1$.
The convergence power spectrum gives constraints on $\sigma_8$ that are degenerate with the matter density parameter $\Omega_{\rm m}$: the power spectrum at small $k$ increases with an increase in both $\Omega_{\rm m}$ or the  $\sigma_8$ normalisation.

Significant second order contributions to the observed two-point statistics are reduced shear \citep{dodelson2006,shapiro2009}, source clustering  and  magnification  \citep{Schneider2002, Schmidt2009} and the deflection of source positions \citep{seljak96, dodelson08}.
The impact of these higher order effects is verified to be negligible at the precision of this analysis, with the derivation and computation of the contributions accounted in \citet{y3-generalmethods}.

\begin{table}
    \caption{Summary of cosmological, systematic, and astrophysical sampling parameters used in the fiducial analysis and their priors. In the case of flat priors, the prior bound to the range indicated in the Value column while Gaussian priors are described by their mean and 1$\sigma$ width.}   
    \label{tab:priors}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{cccc}
Parameter & Symbol & Type & Value \tabularnewline
\hline 
\bf{Cosmological} \tabularnewline
Matter density & $\Omega_m$ & Flat & [0.1, 0.9] \tabularnewline
Baryon density  & $\Omega_b$ & Flat & [0.03, 0.07] \tabularnewline
Scalar spectrum ampl. & $A_s \times 10^{-9}$   & Flat & [0.5, 5.0]\tabularnewline
Hubble parameter & $h$ & Flat & [0.55, 0.91]  \tabularnewline
Spectral ind. & $n_s$ & Flat & [0.87,1.07] \tabularnewline
Neutrino mass & $\Omega_{\nu}h^2$ &  Flat & [0.0006,0.006] \tabularnewline
%Dark energy parameter & $w$ & Fixed & [] \tabularnewline
%\hline 
Curvature  & $\Omega_k$ & Fixed & [0.0] \tabularnewline
Optical depth  & $\tau$ & Fixed & [0.0697] \tabularnewline
\hline 
\bf{Observational} \tabularnewline
Redshift calibration 1 & $\Delta z^1$ & Gauss. & ( 0.0, 0.018 ) \tabularnewline
Redshift calibration 2 &$\Delta z^2$ & Gauss.  & ( 0.0, 0.015 ) \tabularnewline
Redshift calibration 3 &$\Delta z^3$ & Gauss.  & ( 0.0, 0.011 ) \tabularnewline
Redshift calibration 4 &$\Delta z^4$ & Gauss.  & ( 0.0, 0.017 ) \tabularnewline
Shear calibration 1 & $m^1$ & Gauss. & ( -0.006, 0.009 )\tabularnewline
Shear calibration 2 &$m^2$ & Gauss.  & ( -0.020, 0.008 )\tabularnewline
Shear calibration 3 &$m^3$ & Gauss.  & ( -0.024, 0.008 )\tabularnewline
Shear calibration 4 &$m^4$ & Gauss.  & ( -0.037, 0.008 )\tabularnewline
\hline 
\bf{Astrophysical} \tabularnewline
Tidal alignment ampl.                  & $a_1$         & Flat & $[-5,5]$ \tabularnewline
Tidal torque ampl.                  & $a_2$         & Flat & $[-5,5]$ \tabularnewline
Tidal alignment redshift ind.            & $\eta_1$      & Flat & $[-5,5]$ \tabularnewline
Tidal torque redshift ind.             & $\eta_2$      & Flat & $[-5,5]$ \tabularnewline
Tidal alignment bias                       & $b_{\rm ta}$  & Flat & $[0,2]$ \tabularnewline
\hline 
\bf{Shear-ratio} \tabularnewline
Galaxy bias                      & $b_{1-3}$  & Flat & $[0.8,3]$ \tabularnewline
Lens redshifts             & $\Delta z_l^{0}$      & Gauss. & ( 0.006, 0.004 ) \tabularnewline
Lens redshifts             & $\Delta z_l^{1}$      & Gauss. & ( 0.001, 0.003 )  \tabularnewline
Lens redshifts             & $\Delta z_l^{2}$      & Gauss. & ( 0.004, 0.003 )  \tabularnewline
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}


\subsection{Modeling Intrinsic Alignments}

In an idealised case where galaxies' orientation is truly random, the signal detected in $\xi_\pm$ measurements is a purely cosmological one. In reality, astrophysical processes also contribute to the measurements. Dominant among these is an effect known as intrinsic alignment (IA), which arises due to local interactions between galaxies and their environment \citep{hirata04, troxel15, kiessling15}. One can approximate the distortion in a set of galaxies as the sum of intrinsic (I) and cosmological (G) parts $\gamma = \gamma_{\rm I} + \gamma_{\rm G} + \mathcal{\epsilon}_{\rm I}$. Propagated to the two-point functions, the observed E-mode angular power
spectrum is written
\begin{equation}
\begin{split}
\langle \gamma^i \gamma^j \rangle & =
\langle \gamma^i_{\rm G} \gamma^j_{\rm G}\rangle + \langle \gamma^i_{\rm G} \gamma^j_{\rm I}\rangle + \langle \gamma^i_{\rm I} \gamma^j_{\rm G}\rangle + \langle \gamma^i_{\rm I} \gamma^j_{\rm I}\rangle \\
& = C^{ij}_{\rm GG}(\ell) + C^{ij}_{\rm GI}(\ell) + C^{ji}_{\rm GI}(\ell) + C^{ij}_{\rm II}(\ell),
%<\hat{\xi{\pm}}> = \xi_{\pm} + \xi^{\rm II}_{\pm} + \xi^{\rm GI}_{\pm} \,
\end{split}
\end{equation}
\noindent
where, as before, the indices $i,j$ denote redshift bins. The uncorrelated intrinsic $\mathcal{\epsilon}_I$ averages to zero in the limit of many galaxies and does not contribute to the signal (though it does to shape noise, which enters the covariance matrix). In Fourier space, the cosmological term (GG) corresponds to the convergence power spectrum given by Equation~\ref{eq:limber_gg}. The two IA contributions, GI and II, which arise due to correlations between the intrinsic shapes of physically nearby galaxies and intrinsic
correlations between galaxies on neighbouring lines of
sight, respectively, can be written (e.g. \citealt{joachimi10}) as,
\begin{align}\label{eq:limber_giii}
\centering
& {} C_{\rm GI}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{W_i(\chi)\bar{n}_j(\chi)}{\chi^2} \,  C_{\rm GI}\left(\frac{\ell+0.5}{\chi},z(\chi)\right) \\
& C_{\rm II}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{\bar{n}_i(\chi)\bar{n}_j(\chi)}{\chi^2} \,  C_{\rm II}\left(\frac{\ell+0.5}{\chi},z(\chi)\right) \, ,
\end{align}
\noindent
with the kernels as defined previously. 

The fiducial IA model used in the DES Y3 analysis is a nonlinear perturbative prescription, referred to as the Tidal Alignment and Tidal Torquing model (TATT; \citealt{blazek19}). This is motivated by tests on simulated data, detailed \citet{y3-cosmicshear2} and based upon the findings of \citet{samuroff18}.  In brief, the implementation of the TATT model has three contributions and the intrinsic galaxy shape field, $ \gamma^{\rm IA}_{ij}$, measured at the location of source galaxies, can be written as
%governed by amplitudes $C_1$,$C_2$ and $C_{\delta1}$:
\begin{equation}
    \gamma^{\rm IA}_{ij} = \left ( A_1 +  A_{1\delta} \delta \right ) s_{ij} + A_2 s_{ik}s_{kj} + ... \, ,
\end{equation}
\noindent
where $s_{ij}$ is the gravitational tidal field and $\delta$ is the normalised matter overdensity.
This approach captures the `tidal alignment' contribution, linear in the tidal field, such that the first $A_1$ corresponds to the well-studied nonlinear alignment model \citep[NLA][]{catelan01,hirata04,  bridle07} and the second term captures the impact of source density weighting \citep{blazek15}. An additional contribution due to `tidal torquing' \citep{mackey02,codis15}, which is quadratic in the tidal field, is accounted for in the $A_2$ term. 
%TATT model parameters are renormalised (see Section E of  \citet{blazek19}), such that they absorb contributions due to unmodeled small-scale processes. They should thus be considered as effective parameters rather than strictly mapping onto physical alignment mechanisms.

At fixed redshift, the TATT power spectra depend on three amplitude  parameters, an NLA  amplitude, $A_1$, an tidal  torquing  amplitude, $A_2$, and an amplitude for the density weighting term, captured by an effective source linear bias of the galaxies contributing to the tidal alignment signal, $b_{\rm ta}$. The redshift evolution of $A_1$ and $A_2$ is parametrized as a power law, governed by $\eta_1$ and $\eta_2$ -- a  standard  assumption in concurrent NLA analyses. In detail, the prefactors are given by
\begin{align}
  {}&  A_1(z) = -a_1 \bar{C}_1 \frac{\rho_{\rm crit} \Omega_{\rm m}}{D(z)} \left( \frac{1+z}{1+z_0}\right )^{\eta_1}\, , \\
   &  A_2(z) =   5 a_2 \bar{C}_1 \frac{\rho_{\rm crit} \Omega_{\rm m}}{D(z)^2} \left( \frac{1+z}{1+z_0}\right )^{\eta_2}\, , \\
  &  A_{1\delta}(z) = b_{\rm ta} A_1(z)\, ,
\end{align}
\noindent
where a normalization constant, by convention is fixed to $\bar{C}_1=5\times10^{-14} {\rm M}h^{-1}{\rm Mpc}^2$ \citep{brown02}, the pivot redshift is fixed at $z_0=0.62$, following \citet{Troxel2018} and $b_{\rm ta}$ is assumed to be constant in redshift. 


%The full expressions for $P_{\rm GI}$ and $P_{\rm II}$ in terms of $C_1,C_2,C_{1\delta}$ are relatively complicated, and we refer the reader to \citet{blazek19} for details. The various scale dependent terms presented there are computed using \textsc{FAST-PT} \citep{mcewen16,fang17}. It is worth noting that although the GG and GI signals are expected to have no B-mode component by construction, the TATT model does predict non-zero $P^{BB}_{\rm II}$. Although subdominant, the B-mode contributions are propagated to $\xi_+$ and $\xi_-$ in the correct way (Equation \ref{eqn:2ptP} ), and are always included in our modelling unless stated otherwise. 

TATT is a super-space of the more common Nonlinear Alignment (NLA) model \citep{hirata04,bridle07}, such that in the limit $A_2,b_{\rm ta} \rightarrow 0$, TATT reduces to NLA. The NLA has been implemented with some success in the recent past \citep[e.g.][]{Ham20, asgari20} and an extensive comparison to NLA and investigation into the robustness of modelling of this systematic is described in \citet{y3-cosmicshear2}. Given
the sensitivity of IA to the source sample selection and in
the absence of informative priors, the analysis marginalises over the five IA parameters that govern the amplitude and redshift dependence of the signal, $(A_1, A_2, \eta_1, \eta_2, b_{\rm ta})$, with wide flat priors summarised in Table~\ref{tab:priors}.


%The estimator for the two-point shear correlation function does not measure a pure cosmic shear lensing signal. It is contaminated by intrinsic alignments (IA), characterised by
%\begin{equation}
%<\hat{\xi{\pm}}> = \xi_{\pm} + \xi^{\rm II}_{\pm} + \xi^{\rm GI}_{\pm} \, ,
%\end{equation}
%where $\xi^{\rm II}_{\pm}$ estimates the correlation between the intrinsic ellipticities of nearby galaxies and $ \xi^{\rm GI}_{\pm}$ estimates the correlations between the intrinsic ellipticity of a foreground galaxy and the induced shear of a background galaxy. Without modelling and marginalising over the intrinsic alignment contributions to the observed correlation functions, the cosmological signal can be biased. 
%For our fiducial analysis, we model IA with the ..., \\
%Cite Secco et al for details and robustness tests. 


\subsection{Modeling the matter power spectrum and baryonic effects}\label{sec:scalecuts}

\par The impact of baryonic feedback effects on the modelling of the matter power spectrum at small angular scales is a leading systematic uncertainty in the cosmic shear surveys \citep{vandaalen2014, semboloni2013effect, harnois2015baryons}. While feedback processes from Active Galaxy Nuclei (AGN) heat the halo environment and thereby suppresses matter clustering, metalicity can offer cooling channels that conversely enhance clustering power on small scales and these effects depend precisely on redshift and galaxy evolution \citep{semboloni2011quantifying}. Without a successful analytical model to account for this effect, the bias induced can limit the precision of a cosmic shear analysis .

In general, two approaches to mitigate the baryonic bias exist. The exclusion of information from small angular scales to circumvent modelling baryonic feedback. This conservative approach requires investigating the maximum scale up to which plausible models may contaminate, in order to validate the robustness of the modelling for the measurements used in the analysis \citep{Troxel2018}. On the other hand, the impact of the baryonic effect on the matter power spectrum can be accounted for using empirical halo models fitted on hydrodynamic simulations \citep{hildebrandt20, asgari20}, such as \textsc{HMcode} \citep{mead2015}. %Given insufficient knowledge for modelling these effects, the loss of constraining power due to the uncertainty is roughly equivalent to eliminating small-scale information. 

For this DES Y3 analysis adopts the first approach: in order to mitigate biases due to baryonic effects, we employ a DM-only matter power spectrum and limit the analysis to larger angular scales only. A detailed account of this process to define the scale cuts is given in \citet{y3-generalmethods}. In summary, to define a safe angular range for the measurements, it was verified that accounting for any residual impact by marginalizing over baryonic halo model parameters under conservative priors does not bias nor inflate the cosmological parameter constraints. \textsc{HMcode} is used to run a cosmological analysis with two additional halo parameters that capture the baryonic features through the halo concentration, $A$, and the bloating parameter, $\eta_0$. Synthetic cosmic shear data vectors are contaminated with baryonic effects measured from hydrodynamic simulations, according to
\begin{equation}
    P_{\rm NL,b}(k,z) = \frac{P_{\rm hydro}(k,z)}{P_{\rm DMO}(k,z)}P_{\rm NL} (k,z)
\end{equation}
where $P_{\rm hydro}(k,z)$ and $P_{\rm DMO}(k,z)$ are the matter power spectrum measured from hydrodynamic and dark matter only simulations of the same suite. $P_{\rm NL}(k,z)$ is the non-linear matter power spectrum analytically calculated with the \textsc{Halofit} model \citep{smith2003, takahashi2012} with fixed DMO halo parameters. The hydrodynamic simulations from \textsc{EAGLE} \citep{mcalpine} and \textsc{OWLS-AGN} \citep{vanDaalen11} are used as two extreme cases of baryonic feedback effects. The process is repeated with successively less strict scale cuts. Isolating the marginalized posterior in $\Omega_m - S_8$ plane, the threshold is identified where the bias incurred in the contaminated simulated analysis is $<0.3\sigma$, or a $\Delta \chi^2 = 0.5$. 

\citet{y3-generalmethods} finds that bounds of roughly $\theta_+^{\rm min}=2.4$ and $\theta_-^{\rm min}=35.0$ arcmin in $\xi_+$ and $\xi_-$, respectively, satisfies this constraint, with a redshift-dependence as indicated by the grey shaded region in Figure~\ref{fig:xitomo}. Taking these into account, the datavector has 166 and 61 angular bins in  $\xi_+$ and $\xi_-$, and a total of 227 data points. It was concluded that while \textsc{HMcode} demonstrated sufficient protection against baryonic bias, the gain in constraining power from the small-scale measurements is absorbed into the uncertainty on halo parameters, such that eliminating small-scale information was both as constraining and robust for this analysis  \citep{y3-generalmethods}. 


\subsection{Modeling redshift systematics}
\label{sec:modelz}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/DVtomosim_redshift.pdf}
    \label{fig:xitheoryredshift}
    \caption{Impact of uncertainties and choices in redshift calibration on cosmic shear observables. The fiducial simulated $\xi_{\pm}$ signal is shown with $1\sigma$ uncertainty (upper panels, green shaded region) and the fractional difference, with respect to this of an alternative analysis choice is shown in the lower panels, scaled by the statistical uncertainty of the measurements. Shown are the predicted data vectors (i) with the `extreme' \textit{C}-redshift sample ( blue) (ii)  with the `extreme' \textit{MB}-redshift sample (yellow) (iii) without account for the redshift-dependent effects of blending (red). Scale cuts are shown as grey shaded regions.\todo{Add an extreme hyperrank from lower and higher redshift.}\amon{I'm not so sure about this plot.}}
\end{figure*}

An approach previously used for propagating photometric redshift calibration uncertainties into cosmic shear cosmological parameter constraints \citep[e.g.][]{svcosmicshear,Troxel2018,hikage19,asgari20, Ham20} relies on introducing a nuisance parameter $\Delta_z^i$ for the offset of the mean redshift of a each source bin $i$ from its estimate,
\begin{equation}
n_i(z) \rightarrow n_i(z+\Delta_z^i) \, .
\end{equation}

The prior on the $\Delta_z^i$ encapsulates the statistical and systematic calibration uncertainty and can e.g.~be described by a 
Gaussian. This simple way of describing the uncertainty is effective in common scenarios \citep[see][]{Bonnett16}. However, 
uncertainties in the estimated redshift distributions are not limited to the mean redshift, but rather include e.g. the extendedness 
of a redshift distribution's tail. The assumption of a Gaussian prior purely on $\Delta_z^i$ could thus potentially lead to an over- 
or underestimation of the confidence intervals in cosmological parameters, especially as the statistical power of measurement and calibration improves. 

Some studies in the literature have thus chosen to account for uncertainty in the redshift distributions differently than with such a  prior on their mean. For instance, several recent cosmic shear studies by the KiDS collaboration \citep{hildebrandt2017kids, hildebrandt20, joudaki2020} compare cosmological constraints achieved with different redshift calibration strategies, e.g. with different redshift samples, to gauge the uncertainty. 

For DES Y3, we have developed techniques that allow us to marginalize over the full uncertainty of the redshift distribution in a single likelihood analysis, described in the following section.

\subsubsection{\textsc{Hyperrank} and marginalization}

The set of candidate $n(z)$ samples, described in Section~\ref{sec:sompz}, encapsulate the various sources of uncertainty. These samples preserve correlations between tomographic bins, uncertainties on higher order moments of the $n(z)$, and non-Gaussianities in those systematic errors. While the ensemble variance of mean redshift can be expressed as a set of  $\Delta_z^i$ priors, we can choose this fuller accounting for redshift calibration uncertainties instead. 

This alternative to the $\Delta_z^i$ marginalization approach, \textsc{Hyperrank}, is presented in \citet{y3-hyperrank}. Here, a single realization of the $n(z)$s of the four bins is selected in each likelihood evaluation. The sampling across a set of such realizations describes the full uncertainty.

To avoid low sampling efficiency by just selecting a random realization on each evaluation, \textsc{Hyperrank} constructs a mapping between the $n(z)$ ensemble, characterized by a set of descriptive parameters,
%$\mathbf{d}$, 
and a multidimensional grid within a unit hyper-cube.

The coordinates of this cube, $\mathcal{H} \in [0,1)^n$ are then sampled in the MCMC chain. The $n(z)$ realization mapped to the closest grid point to those coordinates is then used in each step.
The set of descriptive parameters
%$\mathbf{d}$ 
must correlate with cosmology so that the posterior varies as smoothly as possible along each of the dimensions of the hyper-cube.
As descriptive values to map realizations, we use the mean redshift $\langle z \rangle_i = \int z\,n_i(z)\,dz$ of the three bins with the largest variance across the realizations of the ensemble.
This corresponds to bins 1, 2 and 4 based on the values from table \ref{tab:priors}. This three-dimensional space provides a significant increase in sampling efficiency over a purely random approach.

Marginalization using \textsc{Hyperrank} preserves the correlation of $n(z)$ variations across redshift and between bins. It is able to correctly propagate uncertainties when the distribution moments are not described by a Gaussian or any other analytical functional form. The impact of redshift uncertainty is tested in Section~\ref{sec:robustredshift}, as well as the robustness of the analysis to using the simple shift parameter, instead of \textsc{Hyperrank}.

\subsubsection{Impact on cosmic shear signal}

Figure~\ref{fig:xitheoryredshift} illustrates the impact of the effects of sources of uncertainty in redshift calibration on the expected cosmic shear data vector. In particular, in blue and red, the predicted measurements with the two `extreme' redshift distributions, calibrated from Cosmos-30 only, $C$, and the maximally-biased $SPC$ sample, $MB$, are shown, compared to the fiducial simulated data vector, with it's $1\sigma$ uncertainty denoted by the shaded green region. The red line indicates the impact of blending effects in the redshift distribution, with a more detailed account of the modelling discussed in Section~\ref{sec:modelm}. Differences are largest in the lowest redshift bin, yet remain below the statistical uncertainty on the basis of an individual data point. As such, the uncertainty due to the choice of redshift sample was limited to encompass only differences between $SC$, $PC$ and $SPC$ distributions. However, due to their coherence across scales and bins, the a likelihood analysis investigating the impact on cosmology with these ensembles is warranted, as explored in Section~\ref{sec:robustredshift}.

\subsection{Modeling shear systematics}\label{sec:modelm}

A residual bias due to multiplicative shear in the DES Y3 catalogue is constrained through measuring the residual bias in shape measurement on simulated data, which relies critically on the fidelity with which the image simulation matches the real data, as summarised in Section~\ref{sec:imsims}. We account for systematic errors in shear estimation in our model for the observed cosmic shear signal. Multiplicative shear bias is commonly modeled as
\begin{equation}
\xi^{ij}_{\rm obs} = (1+m^i)(1+m^j)\xi^{ij} \; ,
\end{equation}
or equivalently as a contribution to the covariance matrix \citep[see e.g.][]{asgari20},
where $m^i$ is defined either globally or per tomographic bin. 

As shown in \citet{y3-imagesims} and described in Section~\ref{sec:imsims}, these multiplicative bias parameters $m^i$ alone do not fully describe the redshift-mixing effect of blending on shear measurements. Rather, to account for blending, the shape of the redshift distributions needs to be modified alongside their normalization.

As our fiducial treatment of shear systematics, we therefore marginalize over joint samples of modifications to the (normalized)  redshift distributions (see \ref{sec:modelz}), as well as multiplicative biases. We assume a model for the correct effective $n_i^{\rm mod}(z)$ for redshift bin $i$ as
\begin{equation}
    n_i^{\rm mod}(z)= [1+F_i(z)]n_i(z) + G_i(z).
\end{equation}
where $F_i(z)$ and $G_i(z)$ are functions of $z$, constrained using image simulations in \citet{y3-imagesims}. They allow for multiplicative and additive deviations from the \mcal response-weighted redshift distribution, $n_i(z)$, presented in Section~\ref{sec:calib}. The term $F_i(z)$ models the impact on the effective weighting of the discrete sources used to construct $n_i(z)$, such as (possibly redshift dependent) multiplicative bias effects. The term $G_i(z)$ captures responses to shear of light at redshifts other than that of the primary galaxy of a detection, due to blending of that primary galaxy with galaxies at different redshifts. The impact of this modification to the $n(z)$ on the shear correlation functions is demonstrated in Figure~\ref{fig:xitheorytomo}. The shear calibration priors per tomographic bin, $m_i$, are listed in Table~\ref{tab:datastats}.

%\todo{ this isn't clear, but it's meant to summarise the systematic (and statistic) uncertainty that went into these samples.} A mixture model method choice incorporates two alternatives to parametrise the $F(z)$ and $G(z)$ model, Smail distribution and a Student's-\textit{t} model. It encompasses variants in the tomographic binning of the simulation, as well as a version that reweights the simulations to better match the properties in the data. 

To demonstrate the importance of this previously not calibrated effect, the analysis is performed without taking into account a redshift-dependent blending impact in Section~\ref{sec:robustshear}.  In such test, the redshift distributions without shear-calibration correction are used with $m$-priors of approximately 0.02 width that represent the impact from masking, detection biases and blending, drawn from \citet[][their Table 3]{y3-imagesims}. Furthermore, we test the impact of the assumption that ignores the correlation between an individual $n(z)$ realisation and the residual multiplicative factor, $m$, at the likelihood-level. To do so the analysis is modified to use \textsc{Hyperrank} but computes the $m$ associated with that realisation, `per-m', as opposed to a global calibration factor.


\begin{comment}
\begin{table}
    \caption{Shear robustness variants}   
    \label{tab:shearrobust}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{ccc}
 & Fiducial & No blending \tabularnewline
\hline 
$m^1$ &  -0.006 $\pm$ 0.009 & -0.013 $\pm$ 0.003 \tabularnewline
$m^2$ & -0.020 $\pm$ 0.008 & -0.018 $\pm$ 0.004 \tabularnewline
$m^3$ & -0.024 $\pm$ 0.008 & -0.023 $\pm$ 0.004  \tabularnewline
$m^4$ &  -0.037 $\pm$ 0.008 & -0.036 $\pm$ 0.006 \tabularnewline
\hline 
$\Delta z^1$ & 0.0 $\pm$ 0.018 & 0.0 $\pm$ 0.016\tabularnewline
$\Delta z^2$ & 0.0 $\pm$ 0.015  & 0.0 $\pm$ 0.013\tabularnewline
$\Delta z^3$ & 0.0 $\pm$ 0.011  & 0.0 $\pm$ 0.006\tabularnewline
 $\Delta z^4$& 0.0 $\pm$ 0.017  & 0.0 $\pm$ 0.015 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}
\end{comment}


\subsection{Aggressive analysis}\label{sec:agg}
The fiducial DES Y3 approach emphasizes conservative modeling choices. In addition to the fidicial analysis, an `aggressive' approach is investigated to demonstrate the potential constraining power of the data. In particular, we alter the aspects of the analysis that would provide significant advancements in precision with more insight: the modelling of intrinsic alignments and the redshift distributions.  In particular, 
\begin{itemize}[itemsep=0pt]
    \item the IA model choice is switched to the more constraining subspace NLA model (with $a_1$ and $\eta_1$)
    \item The $n(z)$ are limited to those from \textit{SPC} only, as our most reliable ensemble, and \textsc{hyperrank} is used to marginalise over an ensemble that captures the uncertainty. 
     \item The redshift-dependent impact of blending of the $n(z)$ and $m$ calibration is neglected. 
\end{itemize}

As these analysis choices do not pass tests on simulated data to recover unbiased cosmology within the prescribed threshold, and therefore are not deemed robust, only the precision to be gained is investigated. The posteriors are centred on the fiducial results.


==> DES cosmic shear 1/table_lcdm.tex <==

\begin{tabular}{lcccccc}
\hline
\hline
\ Data & $S_8$ & $\hat{S}_8$ &$\Omega_{\mathrm{m}}$ & $\sigma_8$ & FoM$_{S_8,\Omega_{\mathrm{m}}}$ & $\chi^2/\mathrm{dof}$ \\ [0.1cm]
\hline
%\renewcommand{\arraystretch}{5.}
\textbf{Fiducial} & $0.759_{-0.023}^{+0.025}$  & 0.755 & $0.290^{+0.039}_{-0.063}$ &  $0.783^{+0.073}_{-0.092}$  & 927 & $237.7/222=1.07$\\

\textbf{$\Lambda$CDM-Optimized} & $  0.772^{+0.018}_{-0.017} $  & 0.774 & $  0.289^{+0.036}_{-0.056} $  & $  0.795^{+0.072}_{-0.076} $  & 1398 & $285.0/268=1.06$
  \\ 
$\Lambda$CDM-Optimized, NLA, fixed neutrino mass & $0.788^{+0.017}_{-0.016}$ & $0.775$ & $0.279^{+0.036}_{-0.053}$ & $0.825^{+0.078}_{-0.79}$ &  1501 & $288.1/270=1.07$ \\

  %\vspace{0.1cm}
{}  &&&& \vspace{0.02cm}  \\
\hline
C$:$ pure photometric sample * & $  0.752^{+0.025}_{-0.024} $  & 0.766  & $  0.303^{+0.043}_{-0.074} $  & $  0.760^{+0.080}_{-0.102} $  & 831 & -
  \\ 
 MB$: $pure spectroscopic sample * & $  0.752^{+0.021}_{-0.025} $ & 0.729 & $  0.298^{+0.042}_{-0.063} $  & $  0.763^{+0.075}_{-0.091} $  & 968 & -
  \\ 
 SOMPZ only & $  0.760^{+0.035}_{-0.031} $ & 0.739 & $  0.292^{+0.043}_{-0.062} $  & $  0.780^{+0.079}_{-0.089} $  & 542 & -
  \\ 
 SOMPZ$+$WZ only & $  0.758^{+0.035}_{-0.028} $  & 0.730 & $  0.298^{+0.044}_{-0.068} $  & $  0.772^{+0.079}_{-0.092} $  & 516 & -
  \\ 
 Alternative lens sample-SR & $  0.768^{+0.021}_{-0.022} $  & 0.757 & $  0.296^{+0.041}_{-0.060} $  & $  0.783^{+0.079}_{-0.091} $  & 1055 & -
  \\ 
 Large-scale-SR & $  0.777^{+0.022}_{-0.023} $ & 0.780 & $  0.331^{+0.043}_{-0.076} $  & $  0.750^{+0.083}_{-0.088} $  & 860 & -
  \\ 
 Hyperrank$:$ full redshift shape model & $  0.755^{+0.023}_{-0.018} $  & 0.744 & $  0.287^{+0.038}_{-0.055} $  & $  0.780^{+0.067}_{-0.082} $  & 1032 & -
  \\ 
 No redshift systematics * & $  0.753^{+0.023}_{-0.023} $ & 0.752 & $  0.271^{+0.032}_{-0.054} $  & $  0.801^{+0.081}_{-0.078} $  & 1111 & -
  \\ 
 No n$(z)$ blending correction & $  0.761^{+0.024}_{-0.022} $  & 0.753 & $  0.283^{+0.036}_{-0.052} $  & $  0.791^{+0.067}_{-0.082} $  & 1091 & -
  \\ 
 Additional shear uncertainty & $  0.759^{+0.023}_{-0.023} $ & 0.758 & $  0.300^{+0.044}_{-0.057} $  & $  0.767^{+0.071}_{-0.088} $  & 971 & -
  \\ 
 No shear systematics * & $  0.743^{+0.026}_{-0.022} $ & 0.7566 & $  0.292^{+0.035}_{-0.059} $  & $  0.764^{+0.073}_{-0.079} $  & 864 & -
  \\ 
 % \vspace{0.1cm}
{} &&&& \vspace{0.02cm} \\
\hline
No observational systematics * & $  0.742^{+0.022}_{-0.021} $  & 0.740 & $  0.272^{+0.036}_{-0.052} $  & $  0.788^{+0.071}_{-0.086} $  & 1104 & -
  \\ 
 Only cosmological parameters * & $  0.756^{+0.019}_{-0.017} $  & 0.753 & $  0.282^{+0.038}_{-0.054} $  & $  0.789^{+0.070}_{-0.082} $  & 1403 & -
  \\ 
 % \vspace{0.1cm}

{\textit{}} &&&& \vspace{0.02cm} \\
%\textit{Data Vector Choices} \tabularnewline
%& \tabularnewline
 \hline
High-$z$: Bins 1,2 removed & $  0.733^{+0.023}_{-0.025} $ & 0.737 & $  0.355^{+0.050}_{-0.080} $  & $  0.683^{+0.069}_{-0.090} $  & 784 & - 
  \\ 
 Low-$z$: Bins 3,4 removed & $  0.750^{+0.045}_{-0.039} $ & 0.806 & $  0.289^{+0.034}_{-0.099} $ &  $  0.787^{+0.144}_{-0.122} $  & 355 & - 
  \\ 
 $\xi_-$ only & $  0.753^{+0.028}_{-0.032} $  & 0.747 & $  0.265^{+0.031}_{-0.061} $  & $  0.812^{+0.090}_{-0.098} $  & 829 & - 
  \\ 
 $\xi_+$ only & $  0.779^{+0.022}_{-0.020} $  & 0.777 & $  0.288^{+0.039}_{-0.062} $  & $  0.805^{+0.081}_{-0.093} $  & 1008 & - 
  \\ 
 Small angular scales & $  0.770^{+0.021}_{-0.021} $  & 0.763 & $  0.283^{+0.039}_{-0.061} $  & $  0.803^{+0.082}_{-0.086} $  & 934 & - 
  \\ 
  
  Large angular scales & $  0.737^{+0.027}_{-0.031} $  & 0.734 & $  0.268^{+0.033}_{-0.054} $  & $  0.790^{+0.079}_{-0.089} $  & 845 & - \\
  %\vspace{0.1cm}
{} &&&& \vspace{0.02cm} \\
\hline
DES Y1 & $0.780^{+0.027}_{-0.021}$ & - & $0.319^{+0.044}_{-0.062}$ & $0.764_{-0.072}^{+0.069}$ & 625 & $227/211 = 1.08$ \\
KiDS-1000 & $0.759^{+0.024}_{-0.021}$ & -  & $0.246^{+0.101}_{-0.060}$ & $0.838^{+0.140}_{-0.141}$ & 650 & $85.5/70.5=1.21$\\
HSC Y1 $C_\ell$ &  $0.780^{+0.030}_{-0.033}$ & - & $0.162^{+0.086}_{-0.044}$ & - & 461 & $45.4/53 = 0.86$ \\
HSC Y1 $\xi_\pm$ & $0.804^{+0.032}_{-0.029}$ & - & $0.346^{+0.052}_{-0.100}$ & $0.766^{+0.110}_{-0.093}$ &  402 & $162.3/167=0.97$ \\
Planck 2018 TT + TE + EE + lowE & $0.827^{+0.019}_{-0.017}$ & - & $0.327^{+0.008}_{-0.017}$  & $0.793^{+0.024}_{-0.009}$ &  3938 & - \\
  \\ 
\hline
\hline
\end{tabular}


==> extra_notneeded/abe/psfextra.tex <==
\begin{comment}
\begin{center} 
 \centering 
 \begin{table}
 \begin{tabular}{ ccccc} \hline 
 & Bin 1 & Bin 2 & Bin 3 & Bin 4 \\ \hline \rule{0pt}{3ex} 
 $\alpha$ & $0.019_{-0.003}^{+0.003}$ & $0.017_{-0.004}^{+0.004}$ & $0.013_{-0.004}^{+0.004}$ & $0.029_{-0.005}^{+0.005}$\\ \rule{0pt}{3ex} 
 $\beta$ & $0.9_{-0.2}^{+0.2}$ & $1.8_{-0.2}^{+0.2}$ & $2.3_{-0.2}^{+0.2}$ & $1.6_{-0.3}^{+0.3}$ \\ \rule{0pt}{3ex} 
 $\eta$ & $-1.8_{-2.3}^{+2.4}$ & $-5.8_{-2.6}^{+2.7}$ & $1.8_{-2.6}^{+2.6}$ & $2.8_{-3.4}^{+3.2}$ \\  \rule{0pt}{3ex} 
 $\chi^{2}$ & $147.0$ & $209.4$ & $203.4$ & $213.0$ \\ 
 $\chi^{2}_{\nu}$ & $1.3$ & $1.8$ & $1.7$ & $1.8$ \\ \hline 
 \end{tabular}
 \label{tab:abe}
 \caption{The values of the parameters $\alpha$,$\beta$ and $\eta$ for each redshift bin, estimated from fits to the mean-substracted $\rho$-statistics, according to equation~\ref{eq:psf}, as well as the (reduced) goodness-of-fit, $\chi^{2}$ ($\chi^{2}_{\nu}$) for $\nu=117$ degrees of freedom. }
 \end{table}
\end{center}
\end{comment}


\begin{comment}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{abe/figs/tau0_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau1_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau2_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau3_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau4_bestfit.png}
\includegraphics[width=0.3\textwidth]{abe/figs/tau5_bestfit.png}
\caption{Best fits of model $\rho(\theta)$ to data $\tau(\theta)$ for the four different redshift bins}
\label{fig:taubestfits}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{abe/figs/xipcont_xipfid_abe_1sig.png}
\includegraphics[width=0.4\textwidth]{abe/figs/ximcont_ximfid_abe_1sig.png}
\caption{\label{fig:xipbias} Comparison of the bias of the shear 2PCF due to PSF additive errors $\delta \xi^{\textrm{PSF}}$ with fiducial 2PCF $\xi$  }
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_a.png}
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_b.png}
\includegraphics[width=0.4\textwidth]{abe/figs/contribution_rhosp_c.png}
\caption{Bias of the shear two-point correlation function in terms of different diagnostics equations }
\caption{\label{fig:rhoscontribution}}
\end{figure}
\end{comment}





%For the $i$-th redshift bin, is expanded to
\begin{comment}
\begin{align}
\label{eq:2pcfbias}
\xi_{\textrm{obs}}^{ij'} &= \xi_{+ t}^{ij'} + \alpha^{i}\alpha^{j} \rho_{0} + \beta^{i}\beta^{j} \rho_{1} + \eta^{i}\eta^{j}\rho_{3} \\
&+ \left(\beta^{i}\alpha^{j} + \beta^{j}\alpha^{i}\right)\rho_{2}+
 \left( \alpha^{i}\eta^{j}+\alpha^{j}\eta^{i} \right)\rho_{5} \\
 &+ \left(\beta^{i}\eta^{j}+\beta^{j}\eta^{i} \right)\rho_{4} 
\end{align}

\end{comment}
%To find this parameters we define the likelihood function
%\begin{equation}
%\mathcal{L}=|C|^{-1/2} \exp\left(-\frac{{\bf d}^T {\bf C}^{-1}{\bf d}}{2}\right),
%\label{eq:likelihoodbebq}
%\end{equation}
%where 
%\begin{equation}
%\begin{aligned}
%    \xi_{p}= \left[ \alpha\rho_{0+}'+\beta\rho_{2+}'+\eta\rho_{5+}', \alpha\rho_{0-}'+\beta\rho_{2-}'+\eta\rho_{5-}', \right.
%    \\
%    \alpha\rho_{2+}'+\beta\rho_{1+}'+\eta\rho_{4+}', \alpha\rho_{2-}'+\beta\rho_{1-}'+\eta\rho_{4-}'), 
%    \\
%    \left. \alpha\rho_{5+}'+\beta\rho_{4+}'+\eta\rho_{3+}', \alpha\rho_{5-}'+\beta\rho_{4-}'+\eta\rho_{3-}' \right],
%\end{aligned}
%\end{equation}
%\begin{equation}
%    \hat{\xi}=\left[\tau_{0+}, \tau_{0-},\tau_{2+}, \tau_{2-},\tau_{5+},\tau_{5-} \right]
%\end{equation}
%and $\bf{C}$ is the covariance matrix of the data vector $\hat{\xi}$. 
%where the $\rho$- statistics  are defined as for galaxy-star fields as $\rho_{0}=\left\langle \pp\pp \right\rangle $, $\rho_1= \left\langle \vqst \vqst \right\rangle$,  $\rho_2= \left\langle \vqst \pp \right\rangle$, $\rho_3= \left\langle \vwst \vwst \right\rangle$, $\rho_4= \left\langle \vqst \vwst \right\rangle$ and $\rho_5= \left\langle  \pp \vwst\right\rangle$. And $\tau_{0}=\left\langle \vecgest \pp\right\rangle$, $\tau_{2}=\left\langle \vecgest \vqst \right\rangle$ and $\tau_5= \left\langle \vecgest \vwst \right\rangle$. %The primed notation in $\rho(\theta)$ means mean substraction for each star field involved. The covariance matrix was obtained using Jackknife sampling. Both $\tau(\theta)$ and $\rho(\theta)$ were meausured using \code{TreeCorr} with 20 logarithmic angular bins from 0.1 arcmin to 250 arcmin.  We solve this problem once for each redshift bin, since our star field is local we need to update only the correlations involving galaxies, i.e, $\tau(\theta)$. To solve the fitting problem we sample the posterior distribution using \code{emcee} \cite{foremanmackey19}. 




==> extra_notneeded/abe/table_abe_margin_eq4_Y3_03-31-20_JKmarco.tex <==
\begin{center} 
 \centering 
 \begin{table}
 \begin{tabular}{ c|c|c|c|c} \hline 
 & \textrm{Bin}1 & \textrm{Bin}2 & \textrm{Bin}3 & \textrm{Bin}4 \\ \hline \rule{0pt}{3ex} 
 $\alpha$ & $0.019_{-0.003}^{+0.003}$ & $0.017_{-0.004}^{+0.004}$ & $0.013_{-0.004}^{+0.004}$ & $0.029_{-0.005}^{+0.005}$\\ \rule{0pt}{3ex} 
 $\beta$ & $0.884_{-0.232}^{+0.230}$ & $1.757_{-0.241}^{+0.232}$ & $2.275_{-0.236}^{+0.241}$ & $1.601_{-0.270}^{+0.280}$ \\ \rule{0pt}{3ex} 
 $\eta$ & $-1.835_{-2.329}^{+2.362}$ & $-5.815_{-2.616}^{+2.656}$ & $1.860_{-2.619}^{+2.618}$ & $2.883_{-3.370}^{+3.190}$ \\  \rule{0pt}{3ex} 
 $\chi^{2}$ & $146.996$ & $209.378$ & $203.418$ & $213.038$ \\ 
 $\chi^{2}_{(\nu=117)}$ & $1.256$ & $1.790$ & $1.739$ & $1.821$ \\ \hline 

 \end{tabular}
 \label{tab:abe}
 \caption{The values of the parameters $\alpha$,$\beta$ and $\eta$ for different tomographic bins, estimated from mean-substracted $\rho(\theta)$ and cross-correlations galaxy-star $\tau(\theta)$). }
 \end{table}
\end{center}


==> extra_notneeded/data.tex <==

\begin{figure*}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figs/DESY3neff.pdf}
  %\captionof{figure}{A figure}
  \label{fig:test1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figs/DESY3meanz.pdf}
  %\captionof{figure}{Another figure}
  \label{fig:test2}
\end{minipage}
\caption{The DES-Y3 footprint showing the variation of the number density across the sky, as determined with the \mcal catalog (left) and the variation in mean redshift of that catalog (right). Overlaid are the locations and the outline of the Y1 footprint (left) and the locations of three of the four DES Deep Fields \citep{y3-deepfields} (right, dark points; the fourth field, invisible here, is COSMOS). The catalog spans an unmasked 4143 deg$^2$ with an average number density of 5.9 arcmin$^{-2}$ and a mean redshift of 0.633. 
}
\label{fig:map}
\end{figure*}

The Dark Energy Survey (DES) has completed a six year observing program at the Cerro Tololo Inter-American Observatory (CTIO), using the 570-megapixel Dark Energy Camera  \citep{flaugher15}. Ultimately, the complete survey spans 5000 square degrees of the Southern hemisphere in the $grizY$ bands with exposure times of 90 seconds in $griz$ and 45 seconds in $Y$ \citep{des-overview}. With 10 overlapping exposures over the full wide-field area, the survey reaches a limiting magnitude of $i \sim 24$.
%\NS{FYI, it is 23.0 for Y3 for SN = 10 extended objects or 23.3 considering fixed apertures at SN = 10. For Y6 it will be closer to 23.8 and 24 respectively I think}.

This DES Year 3 (Y3)  analysis is limited to the the data acquired over the first three years of observations, from August 15, 2013  to February 12, 2016. The survey footprint spans 4946 square degrees, after masking, with a mean depth of four exposures, with depth reaching S/N $\sim10$ for extended objects up to $i_{AB}\sim23.0$ \citep{y3-gold}. The median recorded seeing (FWHM) in the $riz$ bands is  0.98, 0.89, 0.85 arcsec, respectively for the DES Y3 shape catalog. 

The DES Y3 dataset exploits a number of improvements compared to the DES Y1 catalog, including updates in sky-background modeling, better morphological star-galaxy classification and astrometric solutions, reduced photometric residuals compared to Gaia with photometric calibration uniformity down to $< 3$ mmag, the introduction of  per-object chromatic corrections and improvements to the Point-Spread Function (PSF) modelling \citep{y3-piff} and better flagging of imaging artifacts. These improvements, as well as the production and validation of a `Gold’ catalogue of 390 million objects prior are described in detail in \citet{y3-gold}.
\begin{comment}
\begin{table*}
    \caption{c terms. }  
\label{tab:datastats}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{ccc|cc|cc|cc|cc}
%\hline 
Bin $\times 10^{-4}$& $ w e_1 $  & $w e_2 $ & $e_1 $  & $e_2 $ & Y1 $e_1$ & Y1 $e_2$&  Y3, Y1 area $e_1$&  Y3, Y1 area $e_2$ &  Y3, Y1 area $w e_1$&  Y3, Y1 area $w  e_2$    \tabularnewline
\hline 

0 & 3.22 & 1.60 & 3.50 & 1.58 & 0.8 & 4.3 & 2.76 & 1.87 \tabularnewline
1 & 3.36 & 0.38 & 3.51 & 0.77  & 1.6 & 4.5& 2.35 & 1.26 \tabularnewline
2 & 3.77 & 0.07 & 3.94 & 0.29 & 3.8 & -2.0 & 3.59 & -1.55 \tabularnewline
3 & 4.06 & -0.27 & 4.54 & -0.06 & 8.9 & -1.7 & 4.85 & -1.36 \tabularnewline
%\hline 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table*}
\end{comment}



\subsection{Shape measurement}
%\label{sect:cat_selection}
Shape measurement can be summarised with a first-order approximation of the observed ellipticity or shear estimator, $\epsilon^{\rm obs}$, of the form
\begin{equation}
\label{eqn:shearbias}
    \epsilon^{\rm obs} = (1+m)(\epsilon^{\rm int} + \gamma) + c\, ,
\end{equation}
where the intrinsic ellipticity of the galaxy, $\epsilon^{\rm int}$ has an additional cosmic shear, $\gamma$, as well as an additive bias, $c$, and multiplictive bias, $m$.

For the DES Y3 analysis, \mcal is used to produce the shear catalog \citep{SheldonMcal2017, Huff_Mandelbaum_2017}. This method calibrates shear statistics, such as a mean shear estimate or the shear two-point function, from available imaging data, without reliance on prior information about galaxy properties. 
It measures the ellipticity using a single Gaussian model that is fit to each detected object, for all the available epochs, using the $riz$-band images (the $g$-band is excluded in the fit due to insufficient PSF modeling, as detailed in \citet{y3-piff}). During the fit, light from neighbouring objects is masked in order to reduce blending effects. The galaxy image is then deconvolved with the PSF, artificially sheared, reconvolved by a symmetrized version of the PSF and the ellipticity remeasured. Done repeatedly, this results in one unsheared and four sheared versions of the shape catalog (one for each direction ($\pm$) and component of shear), each of which include unique flux measurements, to construct the shear response matrix, \mcalRg, via numerical derivatives of the ellipticity.  The response matrix is a noisy quantity on a single galaxy basis, but ensemble averages are unbiased and known to a high degree of accuracy given the size of the DES Y3 sample. The pipeline is largely based upon that used in the DES Y1 analysis the inclusion of an inverse variance weighting for the galaxies, employed to boost the signal-to-noise of the data. The details of this implementation can be found in \citet{y3-shapecatalog}. 

The \mcal\ pipeline is designed to self-calibrate biases in the shear estimation by correcting for not only the response of the shear estimator, but also the selection biases \citep{Huff_Mandelbaum_2017}. The artificially sheared versions of each original galaxy image are used to compute the shear response matrix, using a central finite difference estimate. Selection biases can be corrected for by selecting objects on sheared measurements and computing a selection response, \mcalRs,  as, 
 \begin{eqnarray}
\left<\mcalRs_{i,j} \right>  = \frac{\left< e_i\right>^{S_+}-\left< e_i\right>^{S_-}}{\Delta \gamma_j} \, ,
\end{eqnarray}
where $\left<e_i\right>^{S_+}$ represents the mean of the $i$th ellipticity component measured on images without applied shearing in component $j$, over the group of galaxies selected using the parameters extracted from positively sheared images. $\left<e_i\right>^{S_-}$ is the analogue quantity for negatively sheared images. To calibrate the mean shear of the catalog, it is sufficient to consider the total response matrix:
\begin{eqnarray}
\label{eqn:response}
\left<\boldsymbol{R} \right> =  \left<\boldsymbol{R}_\gamma \right> + \left<\boldsymbol{R}_S \right> \, .
\end{eqnarray}
 The response matrix is diagonal, within a very good approximation and as a consequence, the mean shear response correction reduces to element-wise division. The \mcal\ response accounts for shear biases at a level of a few parts in a thousand in absence of blends and detection biases \citep{SheldonMcal2017}.  The current \mcal\ implementation, however, does not correct for a shear-dependent detection bias \citep{metadetect}, which leaves a multiplicative factor at the level of $m\sim2-3$\% and it is calibrated using image simulations in \citep{y3-imagesims} and discussed in Section~\ref{sec:imsims}. 



\subsection{DES Y3 weak lensing catalog and validation}

Only objects that pass a number of criteria are included in the weak lensing selection. This is encoded in a \texttt{INDEX/SELECT} column in the catalog and encompasses selections based on a combination of galaxy and PSF properties, which are designed to reduce potential systematic biases due to, for example blending, PSF mis-estimation and stellar contamination. In addition, magnitude selections are imposed ($i=18-23.5$ and $rz=15-26$) to limit the analysis to include only galaxies with robust redshift estimation. Finally, we limit our study to objects that are contained within the redMaGiC mask, bringing the footprints' final effective area to span $A_{\rm eff}= 4143$ deg$^2$.  The resulting \mcal\ catalog yields 100 202 538 objects, with a weighted number density of $n_{\rm eff}=5.90$ galaxies arcmin$^{-2}$, as defined by \cite{Heymans13}, spanning a final area of $A_{\rm eff}= 4143$ deg$^2$ . Table~\ref{tab:datastats} lists the effective number density for the full catalog and the corresponding weighted ellipticity variance.  The statistical power of the \mcal\ catalog without galaxy weights is tripled compared to Y1, with weighting increasing this further by $\approx 25\%$ \cite{y3-shapecatalog}. 

The spatial variation of number density over the survey footprint is shown in the left-hand panel of Figure~\ref{fig:map} with a map that utilises \texttt{SKYMAPPER}\footnote{https://github.com/kadrlica/skymap} in \textsc{HEALPIX} cells of nside=1024. Overlaid are the bounds of the previous DES Y1 and SV surveys.

The \mcal\ shape catalog has passed a raft of empirical tests detailed in \citet{y3-shapecatalog}, aimed at identifying residual additive biases for the full catalog. These validated against systematic errors connected to PSF errors, which were proven to be negligible for the full catalog with a smaller amplitude compared to the DES Y1 analysis. In addition, the catalog was proven robust against the presence of spurious B-modes using two different estimators, COSEBIs and Pseudo-$C_\ell$, which consistently resulted in a null detection (see also Appendix~\ref{App:Bmodes}). In Section~\ref{sec:robustshear}, these tests are extended to the tomographic case. Further tests included checking the dependency of the two components of the shear with respect to a number of galaxy or survey properties, finding no significant correlations, except for a linear dependence between $\langle e_1 \rangle$ and the ratio between the galaxy size and PSF size. The origin of this trend is unknown, but it was verified to be safely neglected in the cosmological analysis.



 
\begin{table*}
    \caption{DES Y3 data properties per redshift bin: the unweighted number of objects passing the weak-lensing selection, the effective number density $n_{\rm eff}$ (gal/arcmin$^2$), calculated with $A_{\rm eff}= 4143$ deg$^2$, the per-component shape noise, $\sigma_e$, the mean redshift, $z_{\rm mean}$, the spread in the mean redshift of the redshift distribution realisations, $\Delta z$, the shear calibration parameter, $m$, and the mean shear per component, $c_{1,2}=\langle e_{1,2} \rangle$. }  
\label{tab:datastats}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{cccccccccccc}
%\hline 
Redshift bin & no. objects & $n_{\rm eff}$ & $\sigma_e$ &  $z_{\rm mean}$  & $\langle e_1 \rangle \times 10^{4}$  & $\langle e_2 \rangle \times 10^{4}$ & $\Delta z$& $m$ & $\Delta z_{\rm no blend}$& $m_{\rm no blend}$   \tabularnewline
\hline 
Full & 100 204 026 &5.900 & 0.268 &  0.633 &  - & -  & - & - & - & - \tabularnewline
0 & 24 941 833 & 1.476 & 0.243 & 0.336 & 3.22 & 1.60  &    0.018 & -0.006 $ \pm $ 0.009 & 0.016  & -0.013 $ \pm $ 0.003\tabularnewline
1 & 25 281 777 & 1.479 & 0.262 & 0.521 & 3.36 & 0.38 &  0.015 & -0.020 $ \pm $ 0.008 & 0.013  & -0.018 $ \pm $ 0.004\tabularnewline
2 & 24 892 990 & 1.484 &  0.259 &  0.742 & 3.77 & 0.07&  0.011 & -0.024 $ \pm $ 0.008 & 0.006  & -0.023 $ \pm $ 0.004 \tabularnewline
3 & 25 092 344 & 1.461 & 0.301 &  0.964  & 4.06 & -0.27 &  0.017 & -0.037 $ \pm $ 0.008 & 0.015  & -0.036 $ \pm $ 0.006 \tabularnewline
%\hline 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table*}

==> extra_notneeded/modelling.tex <==
In this section, we outline the baseline theoretical model for the shear 2-point correlation functions used in this analysis and discuss the evidence for its robustness. That is, it is exemplified in \citep{y3-generalmethods} that systematic errors in the model are subdominant to the precision of the data, in order to derive unbiased cosmological parameters. 

For parameter inference, the likelihood, $\mathcal{L}(\textbf{p})$, is assumed to be a multivariate Gaussian in the multi-dimensional parameter space,
\begin{equation}
\ln{\mathcal{L}(\textbf{p})} = -\frac{1}{2} \sum_{ij} (D_i-T_i(\textbf{p})\,\,C^{-1}_{ij}\,\,(D_j-T_j(\textbf{p})) \,,
\end{equation}
where $\textbf{p}$ denotes the full set of parameters. The data vector, $D$, presented in Section~\ref{sec:measurement} initially contains 20 angular data points over 4 redshift bins and 2 correlation functions, which amounts to
227 data points after the limiting the angular scales, according to Section~\ref{sec:scalecuts}. $D_i$ represents the $i$th element of the data vector, comprised of the tomographic two-point correlation functions,  $\xi_{\pm}$, presented in Figure~\ref{fig:xitomo}. the corresponding theoretical prediction for the measurements,  $T_i(\textbf{p})$, are detailed in this section. The covariance matrix, $C$, summarised in Section~\ref{sec:covariance}, does depend on the model parameters $\textbf{p}$, but a fiducial set of parameters is assumed and use a fixed covariance implemented in this analysis, after an iterative process. The posteriors of the cosmological parameters are computed as the product of the likelihood with the priors, $\mathcal{P(\textbf{p})}$, listed in Table~\ref{tab:priors}. 

The likelihood is sampled with the \textsc{Polychord sampler} \cite{Handley15}. This analysis pipeline is built upon the framework \textsc{CosmoSIS} \citep{zuntz15}, a modular cosmological parameter estimation code. Although the fiducial settings (500 live points, tolerance 0.1) have been
tested to demonstrate the accuracy of the posteriors and Bayesian evidence estimates \citep[see][]{Lemos2020}, the position of the peak in 19 dimensional space is noisy. As such, point estimates, are obtained with the \textsc{MaxLike} minimizer. Validation of this aspect is achieved through redundancy in an implementation of the analysis pipeline independently in \textsc{cosmolike} \citep{Krause17,y3-generalmethods}. To calculate the linear matter power spectrum $P_{\rm NL}(k, z)$, \textsc{CosmoSIS} uses \textsc{CAMB} \citep{CAMB}.  


Cosmological, astrophysical, and systematic parameters are constrained for the $\Lambda$CDM model. For the case of cosmological parameters that are not well-constrained by cosmic shear, informative priors that widely encompass allowed values from external experiments are used. In
particular, for $\Omega_{\nu}h^2$ we take a lower limit derived from oscillation experiments [105], and an upper limit  that is roughly five times the 95\% confidence limit of the limiting value found by external data,  $\Omega_{\nu}h^2 \sim 0.002$ \citep{Planck2018}. These prior boundaries are reported in Table~\ref{tab:priors}. We leave exploration of other cosmological models to future work. In this section, we detail the fiducial cosmological model used in the analysis, as well as the modelling of the systematics. 



\subsection{Cosmic shear signal}
\begin{comment}
\begin{equation}
\centering
\xi^{ij}_{+}(\theta) = \frac{1}{2 \pi} \int d\ell \,\,\, \ell P_{\kappa}^{ij}(\ell)  \, J_{0}(\ell\theta) 
\end{equation}
\begin{equation}
\centering
P_{\kappa}^{ij}(\ell) = \int d\chi \,\,\,  Q(\chi) \, P_{\delta}\big(\frac{\ell}{\chi},\chi\big) 
\end{equation}
\end{comment}
The observed angular two-point correlation for two redshift bins, $i$ and $j$, is theoretically expressed in terms of the the convergence power spectrum, $C_{\kappa}(\ell)$, at an angular wavenumber, $\ell$, as
\begin{align}
\centering
\label{eqn:2ptP}
{}& \xi_+(\theta) = \sum_{\ell} \frac{2\ell+1}{4\pi} G^\pm_\ell(\cos \theta) \qty[C_{\kappa,\textrm{EE}}^{ij}(\ell)\pm C_{\kappa, \textrm{BB}}^{ij}(\ell)] \, , \\
& \xi_-(\theta) = \sum_{\ell} \frac{2\ell+1}{4\pi} G^\pm_\ell(\cos \theta) \qty[C_{\kappa,\textrm{EE}}^{ij}(\ell) - C_{\kappa, \textrm{BB}}^{ij}(\ell)],
\end{align}
\noindent
where the functions $G^\pm_\ell(x)$ are computed from Legendre polynomials $P_\ell(x)$ (see, e.g. \citealt{y3-covariances}, appendix A). We include the B-mode power spectra here for completeness. Although cosmological lensing does not produce B-modes, our fiducial model does include a B-mode contribution from intrinsic alignments, and so we show the more general expression here.  

The 2D convergence power spectrum, $C_{\kappa}$, can be related to the non-linear 3D matter power spectrum, $P_{\delta}$, via a simplification with a flat-sky and  the Limber approximation \citep{Limber53,Limber_LoVerde2008}.  These approximations begin to break down for small $\ell$-modes. The applicability of these approximations and corrections are investigated in \citet{Kilbinger17} and \cite{Kitching17} and a `hybrid' case, used in most recent cosmic shear analyses, can be written as, 
\begin{equation}
\centering
C_{\kappa}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{W_i(\chi)W_j(\chi)}{\chi^2}  P_{\delta}\left(k=\frac{\ell+0.5}{z(\chi)},\chi\right) \, ,
\end{equation}\label{eq:limber_gg}
\noindent
where $\chi_{\rm H}$ is the horizon distance and a flat spatial geometry is assumed, so that $f_K(\chi)$, the comoving angular diameter distance, is simplified to $\chi$. The lensing efficiency kernel, $W_i(\chi)$, for the tomographic bin $i$ is defined as,
\begin{equation}
\label{eqn:kernel}
\centering
W_i(\chi)= \frac{3H_0^2\Omega_{\rm m}}{2c^2}\frac{\chi}{a(\chi)} \int_{\chi}^{\chi_{\rm H}} d\chi' \, \tilde{n}_i(\chi') \frac{\chi'-\chi}{\chi'}  \, ,
\end{equation}
\noindent
where $\tilde{n}_i(\chi) d\chi$ is the effective number of galaxies in $d\chi$ in the $i$th redshift bin, normalised such that $\int_{\chi}^{\chi_{\rm H}} \tilde{n}_i(\chi) d\chi =1$.
The convergence power spectrum gives constraints on $\sigma_8$ that are degenerate with the matter density parameter $\Omega_{\rm m}$: the power spectrum at small $k$ increases with an increase in both $\Omega_{\rm m}$ or the  $\sigma_8$ normalisation.

Significant second order contributions to the observed two-point statistics are reduced shear \citep{dodelson2006,shapiro2009}, source clustering  and  magnification  \citep{Schneider2002, Schmidt2009} and the deflection of source positions \citep{seljak96, dodelson08}.
The impact of these higher order effects is verified to be negligible at the precision of this analysis, with the derivation and computation of the contributions accounted in \citet{y3-generalmethods}.

\begin{table}
    \caption{Summary of cosmological, systematic, and astrophysical sampling parameters used in the fiducial analysis and their priors. In the case of flat priors, the prior bound to the range indicated in the Value column while Gaussian priors are described by their mean and 1$\sigma$ width.}   
    \label{tab:priors}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{cccc}
Parameter & Symbol & Type & Value \tabularnewline
\hline 
\bf{Cosmological} \tabularnewline
Matter density & $\Omega_m$ & Flat & [0.1, 0.9] \tabularnewline
Baryon density  & $\Omega_b$ & Flat & [0.03, 0.07] \tabularnewline
Scalar spectrum ampl. & $A_s \times 10^{-9}$   & Flat & [0.5, 5.0]\tabularnewline
Hubble parameter & $h$ & Flat & [0.55, 0.91]  \tabularnewline
Spectral ind. & $n_s$ & Flat & [0.87,1.07] \tabularnewline
Neutrino mass & $\Omega_{\nu}h^2$ &  Flat & [0.0006,0.006] \tabularnewline
%Dark energy parameter & $w$ & Fixed & [] \tabularnewline
%\hline 
Curvature  & $\Omega_k$ & Fixed & [0.0] \tabularnewline
Optical depth  & $\tau$ & Fixed & [0.0697] \tabularnewline
\hline 
\bf{Observational} \tabularnewline
Redshift calibration 1 & $\Delta z^1$ & Gauss. & ( 0.0, 0.018 ) \tabularnewline
Redshift calibration 2 &$\Delta z^2$ & Gauss.  & ( 0.0, 0.015 ) \tabularnewline
Redshift calibration 3 &$\Delta z^3$ & Gauss.  & ( 0.0, 0.011 ) \tabularnewline
Redshift calibration 4 &$\Delta z^4$ & Gauss.  & ( 0.0, 0.017 ) \tabularnewline
Shear calibration 1 & $m^1$ & Gauss. & ( -0.006, 0.009 )\tabularnewline
Shear calibration 2 &$m^2$ & Gauss.  & ( -0.020, 0.008 )\tabularnewline
Shear calibration 3 &$m^3$ & Gauss.  & ( -0.024, 0.008 )\tabularnewline
Shear calibration 4 &$m^4$ & Gauss.  & ( -0.037, 0.008 )\tabularnewline
\hline 
\bf{Astrophysical} \tabularnewline
Tidal alignment ampl.                  & $a_1$         & Flat & $[-5,5]$ \tabularnewline
Tidal torque ampl.                  & $a_2$         & Flat & $[-5,5]$ \tabularnewline
Tidal alignment redshift ind.            & $\eta_1$      & Flat & $[-5,5]$ \tabularnewline
Tidal torque redshift ind.             & $\eta_2$      & Flat & $[-5,5]$ \tabularnewline
Tidal alignment bias                       & $b_{\rm ta}$  & Flat & $[0,2]$ \tabularnewline
\hline 
\bf{Shear-ratio} \tabularnewline
Galaxy bias                      & $b_{1-3}$  & Flat & $[0.8,3]$ \tabularnewline
Lens redshifts             & $\Delta z_l^{0}$      & Gauss. & ( 0.006, 0.004 ) \tabularnewline
Lens redshifts             & $\Delta z_l^{1}$      & Gauss. & ( 0.001, 0.003 )  \tabularnewline
Lens redshifts             & $\Delta z_l^{2}$      & Gauss. & ( 0.004, 0.003 )  \tabularnewline
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}


\subsection{Modeling Intrinsic Alignments}

In an idealised case where galaxies' orientation is truly random, the signal detected in $\xi_\pm$ measurements is a purely cosmological one. In reality, astrophysical processes also contribute to the measurements. Dominant among these is an effect known as intrinsic alignment (IA), which arises due to local interactions between galaxies and their environment \citep{hirata04, troxel15, kiessling15}. One can approximate the distortion in a set of galaxies as the sum of intrinsic (I) and cosmological (G) parts $\gamma = \gamma_{\rm I} + \gamma_{\rm G} + \mathcal{\epsilon}_{\rm I}$. Propagated to the two-point functions, the observed E-mode angular power
spectrum is written
\begin{equation}
\begin{split}
\langle \gamma^i \gamma^j \rangle & =
\langle \gamma^i_{\rm G} \gamma^j_{\rm G}\rangle + \langle \gamma^i_{\rm G} \gamma^j_{\rm I}\rangle + \langle \gamma^i_{\rm I} \gamma^j_{\rm G}\rangle + \langle \gamma^i_{\rm I} \gamma^j_{\rm I}\rangle \\
& = C^{ij}_{\rm GG}(\ell) + C^{ij}_{\rm GI}(\ell) + C^{ji}_{\rm GI}(\ell) + C^{ij}_{\rm II}(\ell),
%<\hat{\xi{\pm}}> = \xi_{\pm} + \xi^{\rm II}_{\pm} + \xi^{\rm GI}_{\pm} \,
\end{split}
\end{equation}
\noindent
where, as before, the indices $i,j$ denote redshift bins. The uncorrelated intrinsic $\mathcal{\epsilon}_I$ averages to zero in the limit of many galaxies and does not contribute to the signal (though it does to shape noise, which enters the covariance matrix). In Fourier space, the cosmological term (GG) corresponds to the convergence power spectrum given by Equation~\ref{eq:limber_gg}. The two IA contributions, GI and II, which arise due to correlations between the intrinsic shapes of physically nearby galaxies and intrinsic
correlations between galaxies on neighbouring lines of
sight, respectively, can be written (e.g. \citealt{joachimi10}) as,
\begin{align}\label{eq:limber_giii}
\centering
& {} C_{\rm GI}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{W_i(\chi)\bar{n}_j(\chi)}{\chi^2} \,  C_{\rm GI}\left(\frac{\ell+0.5}{\chi},z(\chi)\right) \\
& C_{\rm II}^{ij}(\ell) = \int_0^{\chi_{\rm H}} d\chi \,  \frac{\bar{n}_i(\chi)\bar{n}_j(\chi)}{\chi^2} \,  C_{\rm II}\left(\frac{\ell+0.5}{\chi},z(\chi)\right) \, ,
\end{align}
\noindent
with the kernels as defined previously. 

The fiducial IA model used in the DES Y3 analysis is a nonlinear perturbative prescription, referred to as the Tidal Alignment and Tidal Torquing model (TATT; \citealt{blazek19}). This is motivated by tests on simulated data, detailed \citet{y3-cosmicshear2} and based upon the findings of \citet{samuroff18}.  In brief, the implementation of the TATT model has three contributions and the intrinsic galaxy shape field, $ \gamma^{\rm IA}_{ij}$, measured at the location of source galaxies, can be written as
%governed by amplitudes $C_1$,$C_2$ and $C_{\delta1}$:
\begin{equation}
    \gamma^{\rm IA}_{ij} = \left ( A_1 +  A_{1\delta} \delta \right ) s_{ij} + A_2 s_{ik}s_{kj} + ... \, ,
\end{equation}
\noindent
where $s_{ij}$ is the gravitational tidal field and $\delta$ is the normalised matter overdensity.
This approach captures the `tidal alignment' contribution, linear in the tidal field, such that the first $A_1$ corresponds to the well-studied nonlinear alignment model \citep[NLA][]{catelan01,hirata04,  bridle07} and the second term captures the impact of source density weighting \citep{blazek15}. An additional contribution due to `tidal torquing' \citep{mackey02,codis15}, which is quadratic in the tidal field, is accounted for in the $A_2$ term. 
%TATT model parameters are renormalised (see Section E of  \citet{blazek19}), such that they absorb contributions due to unmodeled small-scale processes. They should thus be considered as effective parameters rather than strictly mapping onto physical alignment mechanisms.

At fixed redshift, the TATT power spectra depend on three amplitude  parameters, an NLA  amplitude, $A_1$, an tidal  torquing  amplitude, $A_2$, and an amplitude for the density weighting term, captured by an effective source linear bias of the galaxies contributing to the tidal alignment signal, $b_{\rm ta}$. The redshift evolution of $A_1$ and $A_2$ is parametrized as a power law, governed by $\eta_1$ and $\eta_2$ -- a  standard  assumption in concurrent NLA analyses. In detail, the prefactors are given by
\begin{align}
  {}&  A_1(z) = -a_1 \bar{C}_1 \frac{\rho_{\rm crit} \Omega_{\rm m}}{D(z)} \left( \frac{1+z}{1+z_0}\right )^{\eta_1}\, , \\
   &  A_2(z) =   5 a_2 \bar{C}_1 \frac{\rho_{\rm crit} \Omega_{\rm m}}{D(z)^2} \left( \frac{1+z}{1+z_0}\right )^{\eta_2}\, , \\
  &  A_{1\delta}(z) = b_{\rm ta} A_1(z)\, ,
\end{align}
\noindent
where a normalization constant, by convention is fixed to $\bar{C}_1=5\times10^{-14} {\rm M}h^{-1}{\rm Mpc}^2$ \citep{brown02}, the pivot redshift is fixed at $z_0=0.62$, following \citet{Troxel2018} and $b_{\rm ta}$ is assumed to be constant in redshift. 


%The full expressions for $P_{\rm GI}$ and $P_{\rm II}$ in terms of $C_1,C_2,C_{1\delta}$ are relatively complicated, and we refer the reader to \citet{blazek19} for details. The various scale dependent terms presented there are computed using \textsc{FAST-PT} \citep{mcewen16,fang17}. It is worth noting that although the GG and GI signals are expected to have no B-mode component by construction, the TATT model does predict non-zero $P^{BB}_{\rm II}$. Although subdominant, the B-mode contributions are propagated to $\xi_+$ and $\xi_-$ in the correct way (Equation \ref{eqn:2ptP} ), and are always included in our modelling unless stated otherwise. 

TATT is a super-space of the more common Nonlinear Alignment (NLA) model \citep{hirata04,bridle07}, such that in the limit $A_2,b_{\rm ta} \rightarrow 0$, TATT reduces to NLA. The NLA has been implemented with some success in the recent past \citep[e.g.][]{Ham20, asgari20} and an extensive comparison to NLA and investigation into the robustness of modelling of this systematic is described in \citet{y3-cosmicshear2}. Given
the sensitivity of IA to the source sample selection and in
the absence of informative priors, the analysis marginalises over the five IA parameters that govern the amplitude and redshift dependence of the signal, $(A_1, A_2, \eta_1, \eta_2, b_{\rm ta})$, with wide flat priors summarised in Table~\ref{tab:priors}.


%The estimator for the two-point shear correlation function does not measure a pure cosmic shear lensing signal. It is contaminated by intrinsic alignments (IA), characterised by
%\begin{equation}
%<\hat{\xi{\pm}}> = \xi_{\pm} + \xi^{\rm II}_{\pm} + \xi^{\rm GI}_{\pm} \, ,
%\end{equation}
%where $\xi^{\rm II}_{\pm}$ estimates the correlation between the intrinsic ellipticities of nearby galaxies and $ \xi^{\rm GI}_{\pm}$ estimates the correlations between the intrinsic ellipticity of a foreground galaxy and the induced shear of a background galaxy. Without modelling and marginalising over the intrinsic alignment contributions to the observed correlation functions, the cosmological signal can be biased. 
%For our fiducial analysis, we model IA with the ..., \\
%Cite Secco et al for details and robustness tests. 


\subsection{Modeling the matter power spectrum and baryonic effects}\label{sec:scalecuts}

\par The impact of baryonic feedback effects on the modelling of the matter power spectrum at small angular scales is a leading systematic uncertainty in the cosmic shear surveys \citep{vandaalen2014, semboloni2013effect, harnois2015baryons}. While feedback processes from Active Galaxy Nuclei (AGN) heat the halo environment and thereby suppresses matter clustering, metalicity can offer cooling channels that conversely enhance clustering power on small scales and these effects depend precisely on redshift and galaxy evolution \citep{semboloni2011quantifying}. Without a successful analytical model to account for this effect, the bias induced can limit the precision of a cosmic shear analysis .

In general, two approaches to mitigate the baryonic bias exist. The exclusion of information from small angular scales to circumvent modelling baryonic feedback. This conservative approach requires investigating the maximum scale up to which plausible models may contaminate, in order to validate the robustness of the modelling for the measurements used in the analysis \citep{Troxel2018}. On the other hand, the impact of the baryonic effect on the matter power spectrum can be accounted for using empirical halo models fitted on hydrodynamic simulations \citep{hildebrandt20, asgari20}, such as \textsc{HMcode} \citep{mead2015}. %Given insufficient knowledge for modelling these effects, the loss of constraining power due to the uncertainty is roughly equivalent to eliminating small-scale information. 

For this DES Y3 analysis adopts the first approach: in order to mitigate biases due to baryonic effects, we employ a DM-only matter power spectrum and limit the analysis to larger angular scales only. A detailed account of this process to define the scale cuts is given in \citet{y3-generalmethods}. In summary, to define a safe angular range for the measurements, it was verified that accounting for any residual impact by marginalizing over baryonic halo model parameters under conservative priors does not bias nor inflate the cosmological parameter constraints. \textsc{HMcode} is used to run a cosmological analysis with two additional halo parameters that capture the baryonic features through the halo concentration, $A$, and the bloating parameter, $\eta_0$. Synthetic cosmic shear data vectors are contaminated with baryonic effects measured from hydrodynamic simulations, according to
\begin{equation}
    P_{\rm NL,b}(k,z) = \frac{P_{\rm hydro}(k,z)}{P_{\rm DMO}(k,z)}P_{\rm NL} (k,z)
\end{equation}
where $P_{\rm hydro}(k,z)$ and $P_{\rm DMO}(k,z)$ are the matter power spectrum measured from hydrodynamic and dark matter only simulations of the same suite. $P_{\rm NL}(k,z)$ is the non-linear matter power spectrum analytically calculated with the \textsc{Halofit} model \citep{smith2003, takahashi2012} with fixed DMO halo parameters. The hydrodynamic simulations from \textsc{EAGLE} \citep{mcalpine} and \textsc{OWLS-AGN} \citep{vanDaalen11} are used as two extreme cases of baryonic feedback effects. The process is repeated with successively less strict scale cuts. Isolating the marginalized posterior in $\Omega_m - S_8$ plane, the threshold is identified where the bias incurred in the contaminated simulated analysis is $<0.3\sigma$, or a $\Delta \chi^2 = 0.5$. 

\citet{y3-generalmethods} finds that bounds of roughly $\theta_+^{\rm min}=2.4$ and $\theta_-^{\rm min}=35.0$ arcmin in $\xi_+$ and $\xi_-$, respectively, satisfies this constraint, with a redshift-dependence as indicated by the grey shaded region in Figure~\ref{fig:xitomo}. Taking these into account, the datavector has 166 and 61 angular bins in  $\xi_+$ and $\xi_-$, and a total of 227 data points. It was concluded that while \textsc{HMcode} demonstrated sufficient protection against baryonic bias, the gain in constraining power from the small-scale measurements is absorbed into the uncertainty on halo parameters, such that eliminating small-scale information was both as constraining and robust for this analysis  \citep{y3-generalmethods}. 


\subsection{Modeling redshift systematics}
\label{sec:modelz}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/DVtomosim_redshift.pdf}
    \label{fig:xitheoryredshift}
    \caption{Impact of uncertainties and choices in redshift calibration on cosmic shear observables. The fiducial simulated $\xi_{\pm}$ signal is shown with $1\sigma$ uncertainty (upper panels, green shaded region) and the fractional difference, with respect to this of an alternative analysis choice is shown in the lower panels, scaled by the statistical uncertainty of the measurements. Shown are the predicted data vectors (i) with the `extreme' \textit{C}-redshift sample ( blue) (ii)  with the `extreme' \textit{MB}-redshift sample (yellow) (iii) without account for the redshift-dependent effects of blending (red). Scale cuts are shown as grey shaded regions.\todo{Add an extreme hyperrank from lower and higher redshift.}\amon{I'm not so sure about this plot.}}
\end{figure*}

An approach previously used for propagating photometric redshift calibration uncertainties into cosmic shear cosmological parameter constraints \citep[e.g.][]{svcosmicshear,Troxel2018,hikage19,asgari20, Ham20} relies on introducing a nuisance parameter $\Delta_z^i$ for the offset of the mean redshift of a each source bin $i$ from its estimate,
\begin{equation}
n_i(z) \rightarrow n_i(z+\Delta_z^i) \, .
\end{equation}

The prior on the $\Delta_z^i$ encapsulates the statistical and systematic calibration uncertainty and can e.g.~be described by a 
Gaussian. This simple way of describing the uncertainty is effective in common scenarios \citep[see][]{Bonnett16}. However, 
uncertainties in the estimated redshift distributions are not limited to the mean redshift, but rather include e.g. the extendedness 
of a redshift distribution's tail. The assumption of a Gaussian prior purely on $\Delta_z^i$ could thus potentially lead to an over- 
or underestimation of the confidence intervals in cosmological parameters, especially as the statistical power of measurement and calibration improves. 

Some studies in the literature have thus chosen to account for uncertainty in the redshift distributions differently than with such a  prior on their mean. For instance, several recent cosmic shear studies by the KiDS collaboration \citep{hildebrandt2017kids, hildebrandt20, joudaki2020} compare cosmological constraints achieved with different redshift calibration strategies, e.g. with different redshift samples, to gauge the uncertainty. 

For DES Y3, we have developed techniques that allow us to marginalize over the full uncertainty of the redshift distribution in a single likelihood analysis, described in the following section.

\subsubsection{\textsc{Hyperrank} and marginalization}

The set of candidate $n(z)$ samples, described in Section~\ref{sec:sompz}, encapsulate the various sources of uncertainty. These samples preserve correlations between tomographic bins, uncertainties on higher order moments of the $n(z)$, and non-Gaussianities in those systematic errors. While the ensemble variance of mean redshift can be expressed as a set of  $\Delta_z^i$ priors, we can choose this fuller accounting for redshift calibration uncertainties instead. 

This alternative to the $\Delta_z^i$ marginalization approach, \textsc{Hyperrank}, is presented in \citet{y3-hyperrank}. Here, a single realization of the $n(z)$s of the four bins is selected in each likelihood evaluation. The sampling across a set of such realizations describes the full uncertainty.

To avoid low sampling efficiency by just selecting a random realization on each evaluation, \textsc{Hyperrank} constructs a mapping between the $n(z)$ ensemble, characterized by a set of descriptive parameters,
%$\mathbf{d}$, 
and a multidimensional grid within a unit hyper-cube.

The coordinates of this cube, $\mathcal{H} \in [0,1)^n$ are then sampled in the MCMC chain. The $n(z)$ realization mapped to the closest grid point to those coordinates is then used in each step.
The set of descriptive parameters
%$\mathbf{d}$ 
must correlate with cosmology so that the posterior varies as smoothly as possible along each of the dimensions of the hyper-cube.
As descriptive values to map realizations, we use the mean redshift $\langle z \rangle_i = \int z\,n_i(z)\,dz$ of the three bins with the largest variance across the realizations of the ensemble.
This corresponds to bins 1, 2 and 4 based on the values from table \ref{tab:priors}. This three-dimensional space provides a significant increase in sampling efficiency over a purely random approach.

Marginalization using \textsc{Hyperrank} preserves the correlation of $n(z)$ variations across redshift and between bins. It is able to correctly propagate uncertainties when the distribution moments are not described by a Gaussian or any other analytical functional form. The impact of redshift uncertainty is tested in Section~\ref{sec:robustredshift}, as well as the robustness of the analysis to using the simple shift parameter, instead of \textsc{Hyperrank}.

\subsubsection{Impact on cosmic shear signal}

Figure~\ref{fig:xitheoryredshift} illustrates the impact of the effects of sources of uncertainty in redshift calibration on the expected cosmic shear data vector. In particular, in blue and red, the predicted measurements with the two `extreme' redshift distributions, calibrated from Cosmos-30 only, $C$, and the maximally-biased $SPC$ sample, $MB$, are shown, compared to the fiducial simulated data vector, with it's $1\sigma$ uncertainty denoted by the shaded green region. The red line indicates the impact of blending effects in the redshift distribution, with a more detailed account of the modelling discussed in Section~\ref{sec:modelm}. Differences are largest in the lowest redshift bin, yet remain below the statistical uncertainty on the basis of an individual data point. As such, the uncertainty due to the choice of redshift sample was limited to encompass only differences between $SC$, $PC$ and $SPC$ distributions. However, due to their coherence across scales and bins, the a likelihood analysis investigating the impact on cosmology with these ensembles is warranted, as explored in Section~\ref{sec:robustredshift}.

\subsection{Modeling shear systematics}\label{sec:modelm}

A residual bias due to multiplicative shear in the DES Y3 catalogue is constrained through measuring the residual bias in shape measurement on simulated data, which relies critically on the fidelity with which the image simulation matches the real data, as summarised in Section~\ref{sec:imsims}. We account for systematic errors in shear estimation in our model for the observed cosmic shear signal. Multiplicative shear bias is commonly modeled as
\begin{equation}
\xi^{ij}_{\rm obs} = (1+m^i)(1+m^j)\xi^{ij} \; ,
\end{equation}
or equivalently as a contribution to the covariance matrix \citep[see e.g.][]{asgari20},
where $m^i$ is defined either globally or per tomographic bin. 

As shown in \citet{y3-imagesims} and described in Section~\ref{sec:imsims}, these multiplicative bias parameters $m^i$ alone do not fully describe the redshift-mixing effect of blending on shear measurements. Rather, to account for blending, the shape of the redshift distributions needs to be modified alongside their normalization.

As our fiducial treatment of shear systematics, we therefore marginalize over joint samples of modifications to the (normalized)  redshift distributions (see \ref{sec:modelz}), as well as multiplicative biases. We assume a model for the correct effective $n_i^{\rm mod}(z)$ for redshift bin $i$ as
\begin{equation}
    n_i^{\rm mod}(z)= [1+F_i(z)]n_i(z) + G_i(z).
\end{equation}
where $F_i(z)$ and $G_i(z)$ are functions of $z$, constrained using image simulations in \citet{y3-imagesims}. They allow for multiplicative and additive deviations from the \mcal response-weighted redshift distribution, $n_i(z)$, presented in Section~\ref{sec:calib}. The term $F_i(z)$ models the impact on the effective weighting of the discrete sources used to construct $n_i(z)$, such as (possibly redshift dependent) multiplicative bias effects. The term $G_i(z)$ captures responses to shear of light at redshifts other than that of the primary galaxy of a detection, due to blending of that primary galaxy with galaxies at different redshifts. The impact of this modification to the $n(z)$ on the shear correlation functions is demonstrated in Figure~\ref{fig:xitheorytomo}. The shear calibration priors per tomographic bin, $m_i$, are listed in Table~\ref{tab:datastats}.

%\todo{ this isn't clear, but it's meant to summarise the systematic (and statistic) uncertainty that went into these samples.} A mixture model method choice incorporates two alternatives to parametrise the $F(z)$ and $G(z)$ model, Smail distribution and a Student's-\textit{t} model. It encompasses variants in the tomographic binning of the simulation, as well as a version that reweights the simulations to better match the properties in the data. 

To demonstrate the importance of this previously not calibrated effect, the analysis is performed without taking into account a redshift-dependent blending impact in Section~\ref{sec:robustshear}.  In such test, the redshift distributions without shear-calibration correction are used with $m$-priors of approximately 0.02 width that represent the impact from masking, detection biases and blending, drawn from \citet[][their Table 3]{y3-imagesims}. Furthermore, we test the impact of the assumption that ignores the correlation between an individual $n(z)$ realisation and the residual multiplicative factor, $m$, at the likelihood-level. To do so the analysis is modified to use \textsc{Hyperrank} but computes the $m$ associated with that realisation, `per-m', as opposed to a global calibration factor.


\begin{comment}
\begin{table}
    \caption{Shear robustness variants}   
    \label{tab:shearrobust}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{ccc}
 & Fiducial & No blending \tabularnewline
\hline 
$m^1$ &  -0.006 $\pm$ 0.009 & -0.013 $\pm$ 0.003 \tabularnewline
$m^2$ & -0.020 $\pm$ 0.008 & -0.018 $\pm$ 0.004 \tabularnewline
$m^3$ & -0.024 $\pm$ 0.008 & -0.023 $\pm$ 0.004  \tabularnewline
$m^4$ &  -0.037 $\pm$ 0.008 & -0.036 $\pm$ 0.006 \tabularnewline
\hline 
$\Delta z^1$ & 0.0 $\pm$ 0.018 & 0.0 $\pm$ 0.016\tabularnewline
$\Delta z^2$ & 0.0 $\pm$ 0.015  & 0.0 $\pm$ 0.013\tabularnewline
$\Delta z^3$ & 0.0 $\pm$ 0.011  & 0.0 $\pm$ 0.006\tabularnewline
 $\Delta z^4$& 0.0 $\pm$ 0.017  & 0.0 $\pm$ 0.015 
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}
\end{comment}


\subsection{Aggressive analysis}\label{sec:agg}
The fiducial DES Y3 approach emphasizes conservative modeling choices. In addition to the fidicial analysis, an `aggressive' approach is investigated to demonstrate the potential constraining power of the data. In particular, we alter the aspects of the analysis that would provide significant advancements in precision with more insight: the modelling of intrinsic alignments and the redshift distributions.  In particular, 
\begin{itemize}[itemsep=0pt]
    \item the IA model choice is switched to the more constraining subspace NLA model (with $a_1$ and $\eta_1$)
    \item The $n(z)$ are limited to those from \textit{SPC} only, as our most reliable ensemble, and \textsc{hyperrank} is used to marginalise over an ensemble that captures the uncertainty. 
     \item The redshift-dependent impact of blending of the $n(z)$ and $m$ calibration is neglected. 
\end{itemize}

As these analysis choices do not pass tests on simulated data to recover unbiased cosmology within the prescribed threshold, and therefore are not deemed robust, only the precision to be gained is investigated. The posteriors are centred on the fiducial results.

